A Survey of Table Reasoning with Large Language Models

Table reasoning, which aims to generate the corresponding answer to the question following the user requirement according to the provided table, and optionally a text description of the table, effectively improving the efficiency of obtaining information. Recently, using Large Language Models (LLMs) has become the mainstream method for table reasoning, because it not only significantly reduces the annotation cost but also exceeds the performance of previous methods. However, existing research still lacks a summary of LLM-based table reasoning works. Due to the existing lack of research, questions about which techniques can improve table reasoning performance in the era of LLMs, why LLMs excel at table reasoning, and how to enhance table reasoning abilities in the future, remain largely unexplored. This gap significantly limits progress in research. To answer the above questions and advance table reasoning research with LLMs, we present this survey to analyze existing research, inspiring future work. In this paper, we analyze the mainstream techniques used to improve table reasoning performance in the LLM era, and the advantages of LLMs compared to pre-LLMs for solving table reasoning. We provide research directions from both the improvement of existing methods and the expansion of practical applications to inspire future research.

==> old_bib.tex <==
@inproceedings{2019TabFactA,
 author = {Wenhu Chen and Hongmin Wang and Jianshu Chen and Yunkai Zhang and Hong Wang and Shiyang Li and Xiyou Zhou and William Yang Wang},
 booktitle = {Proc. of ICLR},
 title = {TabFact: A Large-scale Dataset for Table-based Fact Verification},
 year = {2020}
}

@inproceedings{aggarwal-etal-2023-selfconsistency_efficiency,
 author = {Aggarwal, Pranjal  and
Madaan, Aman  and
Yang, Yiming  and
{Mausam}},
 booktitle = {Proc. of EMNLP},
 title = {Let{'}s Sample Step by Step: Adaptive-Consistency for Efficient Reasoning and Coding with {LLM}s},
 year = {2023}
}

@misc{anonymous2023chainoftable,
 archivePrefix = {arXiv},
 author = {Zilong Wang and Hao Zhang and Chun-Liang Li and Julian Martin Eisenschlos and Vincent Perot and Zifeng Wang and Lesly Miculicich and Yasuhisa Fujii and Jingbo Shang and Chen-Yu Lee and Tomas Pfister},
 eprint = {2401.04398},
 primaryClass = {cs.CL},
 title = {Chain-of-Table: Evolving Tables in the Reasoning Chain for Table Understanding},
 year = {2024}
}

@inproceedings{anonymous2023opentab,
 author = {Anonymous},
 booktitle = {Proc. of ICLR},
 title = {OpenTab: Advancing Large Language Models as Open-domain Table Reasoners},
 year = {2023}
}

@inproceedings{anonymous2024minigpt,
 author = {Anonymous},
 booktitle = {Proc. of ICLR},
 title = {Mini{GPT}-4: Enhancing Vision-Language Understanding with Advanced Large Language Models},
 year = {2024}
}

@misc{bian2023hellama,
 archivePrefix = {arXiv},
 author = {Junyi Bian and Xiaolei Qin and Wuhe Zou and Mengzuo Huang and Weidong Zhang},
 eprint = {2311.08896},
 primaryClass = {cs.CL},
 title = {HELLaMA: LLaMA-based Table to Text Generation by Highlighting the Important Evidence},
 year = {2023}
}

@article{binder,
 author = {Zhoujun Cheng and Tianbao Xie and Peng Shi and Chengzu Li and Rahul Nadkarni and Yushi Hu and Caiming Xiong and Dragomir Radev and Mari Ostendorf and Luke Zettlemoyer and Noah A. Smith and Tao Yu},
 journal = {ICLR},
 title = {Binding Language Models in Symbolic Languages},
 year = {2023}
}

@inproceedings{bogin-etal-2019-global_reasoning,
 author = {Bogin, Ben  and
Gardner, Matt  and
Berant, Jonathan},
 booktitle = {Proc. of EMNLP},
 title = {Global Reasoning over Database Structures for Text-to-{SQL} Parsing},
 year = {2019}
}

@inproceedings{bogin-etal-2019-representing_gnn,
 author = {Bogin, Ben  and
Berant, Jonathan  and
Gardner, Matt},
 booktitle = {Proc. of ACL},
 title = {Representing Schema Structure with Graph Neural Networks for Text-to-{SQL} Parsing},
 year = {2019}
}

@misc{bubeck2023sparks_gpt4,
 archivePrefix = {arXiv},
 author = {Sébastien Bubeck and Varun Chandrasekaran and Ronen Eldan and Johannes Gehrke and Eric Horvitz and Ece Kamar and Peter Lee and Yin Tat Lee and Yuanzhi Li and Scott Lundberg and Harsha Nori and Hamid Palangi and Marco Tulio Ribeiro and Yi Zhang},
 eprint = {2303.12712},
 primaryClass = {cs.CL},
 title = {Sparks of Artificial General Intelligence: Early experiments with GPT-4},
 year = {2023}
}

@misc{cai2023toolmakers,
 archivePrefix = {arXiv},
 author = {Tianle Cai and Xuezhi Wang and Tengyu Ma and Xinyun Chen and Denny Zhou},
 eprint = {2305.17126},
 primaryClass = {cs.LG},
 title = {Large Language Models as Tool Makers},
 year = {2023}
}

@inproceedings{cao-etal-2023-api,
 author = {Cao, Yihan  and
Chen, Shuyi  and
Liu, Ryan  and
Wang, Zhiruo  and
Fried, Daniel},
 booktitle = {Proc. of EMNLP},
 title = {{API}-Assisted Code Generation for Question Answering on Varied Table Structures},
 year = {2023}
}

@inproceedings{chang-fosler-lussier-2023-selective_odis,
 author = {Chang, Shuaichen  and
Fosler-Lussier, Eric},
 booktitle = {Proc. of EMNLP Findings},
 title = {Selective Demonstrations for Cross-domain Text-to-{SQL}},
 year = {2023}
}

@inproceedings{chang-jia-2023-data_icl,
 author = {Chang, Ting-Yun  and
Jia, Robin},
 booktitle = {Proc. of ACL},
 title = {Data Curation Alone Can Stabilize In-context Learning},
 year = {2023}
}

@inproceedings{chen-2023-few,
 author = {Chen, Wenhu},
 booktitle = {Proc. of ACL Findings},
 title = {Large Language Models are few(1)-shot Table Reasoners},
 year = {2023}
}

@misc{chu2023cot_survey,
 archivePrefix = {arXiv},
 author = {Zheng Chu and Jingchang Chen and Qianglong Chen and Weijiang Yu and Tao He and Haotian Wang and Weihua Peng and Ming Liu and Bing Qin and Ting Liu},
 eprint = {2309.15402},
 primaryClass = {cs.CL},
 title = {A Survey of Chain of Thought Reasoning: Advances, Frontiers and Future},
 year = {2023}
}

@inproceedings{cot,
 author = {Wei, Jason and Wang, Xuezhi and Schuurmans, Dale and Bosma, Maarten and ichter, brian and Xia, Fei and Chi, Ed and Le, Quoc V and Zhou, Denny},
 booktitle = {Proc. of NeurIPS},
 title = {Chain-of-Thought Prompting Elicits Reasoning in Large Language Models},
 year = {2022}
}

@misc{cui2021documentai,
 archivePrefix = {arXiv},
 author = {Lei Cui and Yiheng Xu and Tengchao Lv and Furu Wei},
 eprint = {2111.08609},
 primaryClass = {cs.CL},
 title = {Document AI: Benchmarks, Models and Applications},
 year = {2021}
}

@inproceedings{dater,
 author = {Ye, Yunhu and Hui, Binyuan and Yang, Min and Li, Binhua and Huang, Fei and Li, Yongbin},
 booktitle = {Proc. of SIGIR},
 title = {Large Language Models Are Versatile Decomposers: Decomposing Evidence and Questions for Table-Based Reasoning},
 year = {2023}
}

@article{dialogue_survey,
 author = {Ni, Jinjie and Young, Tom and Pandelea, Vlad and Xue, Fuzhao and Cambria, Erik},
 journal = {Artif. Intell. Rev.},
 title = {Recent advances in deep learning based dialogue systems: a systematic survey},
 year = {2022}
}

@article{din-sql,
 author = {Mohammadreza Pourreza and Davood Rafiei},
 journal = {CoRR},
 title = {DIN-SQL: Decomposed In-Context Learning of Text-to-SQL with Self-Correction},
 year = {2023}
}

@inproceedings{dou-etal-2022-knowledge-intensive,
 author = {Dou, Longxu  and
Gao, Yan  and
Liu, Xuqi  and
Pan, Mingyang  and
Wang, Dingzirui  and
Che, Wanxiang  and
Zhan, Dechen  and
Kan, Min-Yen  and
Lou, Jian-Guang},
 booktitle = {Proc. of EMNLP},
 title = {Towards Knowledge-Intensive Text-to-{SQL} Semantic Parsing with Formulaic Knowledge},
 year = {2022}
}

@article{ensemble_study,
 author = {Opitz, D. and Maclin, R.},
 journal = {Journal of Artificial Intelligence Research},
 title = {Popular Ensemble Methods: An Empirical Study},
 year = {1999}
}

@inproceedings{flan,
 author = {Longpre, Shayne and Hou, Le and Vu, Tu and Webson, Albert and Chung, Hyung Won and Tay, Yi and Zhou, Denny and Le, Quoc V. and Zoph, Barret and Wei, Jason and Roberts, Adam},
 booktitle = {Proc. of ICML},
 title = {The flan collection: designing data and methods for effective instruction tuning},
 year = {2023}
}

@inproceedings{gan-etal-2021-robustness_Text-to-SQL,
 author = {Gan, Yujian  and
Chen, Xinyun  and
Huang, Qiuping  and
Purver, Matthew  and
Woodward, John R.  and
Xie, Jinxia  and
Huang, Pengsheng},
 booktitle = {Proc. of ACL},
 title = {Towards Robustness of Text-to-{SQL} Models against Synonym Substitution},
 year = {2021}
}

@misc{gao2023dail,
 archivePrefix = {arXiv},
 author = {Dawei Gao and Haibin Wang and Yaliang Li and Xiuyu Sun and Yichen Qian and Bolin Ding and Jingren Zhou},
 eprint = {2308.15363},
 primaryClass = {cs.DB},
 title = {Text-to-SQL Empowered by Large Language Models: A Benchmark Evaluation},
 year = {2023}
}

@misc{gao2024rag_survey,
 archivePrefix = {arXiv},
 author = {Yunfan Gao and Yun Xiong and Xinyu Gao and Kangxiang Jia and Jinliu Pan and Yuxi Bi and Yi Dai and Jiawei Sun and Qianyu Guo and Meng Wang and Haofen Wang},
 eprint = {2312.10997},
 primaryClass = {cs.CL},
 title = {Retrieval-Augmented Generation for Large Language Models: A Survey},
 year = {2024}
}

@inproceedings{globalgnn,
 author = {Liu, Aiwei and Hu, Xuming and Lin, Li and Wen, Lijie},
 booktitle = {Proc. of KDD},
 title = {Semantic Enhanced Text-to-SQL Parsing via Iteratively Learning Schema Linking Graph},
 year = {2022}
}

@inproceedings{gpt3,
 author = {Brown, Tom and Mann, Benjamin and Ryder, Nick and Subbiah, Melanie and Kaplan, Jared D and Dhariwal, Prafulla and Neelakantan, Arvind and Shyam, Pranav and Sastry, Girish and Askell, Amanda and Agarwal, Sandhini and Herbert-Voss, Ariel and Krueger, Gretchen and Henighan, Tom and Child, Rewon and Ramesh, Aditya and Ziegler, Daniel and Wu, Jeffrey and Winter, Clemens and Hesse, Chris and Chen, Mark and Sigler, Eric and Litwin, Mateusz and Gray, Scott and Chess, Benjamin and Clark, Jack and Berner, Christopher and McCandlish, Sam and Radford, Alec and Sutskever, Ilya and Amodei, Dario},
 booktitle = {Proc. of NeurIPS},
 title = {Language Models are Few-Shot Learners},
 year = {2020}
}

@inproceedings{guo-etal-2019-schema_linking,
 author = {Guo, Jiaqi  and
Zhan, Zecheng  and
Gao, Yan  and
Xiao, Yan  and
Lou, Jian-Guang  and
Liu, Ting  and
Zhang, Dongmei},
 booktitle = {Proc. of ACL},
 title = {Towards Complex Text-to-{SQL} in Cross-Domain Database with Intermediate Representation},
 year = {2019}
}

@inproceedings{herzig-etal-2020-tapas,
 author = {Herzig, Jonathan  and
Nowak, Pawel Krzysztof  and
M{\"u}ller, Thomas  and
Piccinno, Francesco  and
Eisenschlos, Julian},
 booktitle = {Proc. of ACL},
 title = {{T}a{P}as: Weakly Supervised Table Parsing via Pre-training},
 year = {2020}
}

@misc{icl-survey,
 archivePrefix = {arXiv},
 author = {Qingxiu Dong and Lei Li and Damai Dai and Ce Zheng and Zhiyong Wu and Baobao Chang and Xu Sun and Jingjing Xu and Lei Li and Zhifang Sui},
 eprint = {2301.00234},
 primaryClass = {cs.CL},
 title = {A Survey on In-context Learning},
 year = {2023}
}

@inproceedings{jiang-etal-2022-omnitab,
 author = {Jiang, Zhengbao  and
Mao, Yi  and
He, Pengcheng  and
Neubig, Graham  and
Chen, Weizhu},
 booktitle = {Proc. of NAACL},
 title = {{O}mni{T}ab: Pretraining with Natural and Synthetic Data for Few-shot Table-based Question Answering},
 year = {2022}
}

@inproceedings{jiang-etal-2023-structgpt,
 author = {Jiang, Jinhao  and
Zhou, Kun  and
Dong, Zican  and
Ye, Keming  and
Zhao, Xin  and
Wen, Ji-Rong},
 booktitle = {Proc. of EMNLP},
 title = {{S}truct{GPT}: A General Framework for Large Language Model to Reason over Structured Data},
 year = {2023}
}

@misc{jin2022survey_tableqa,
 archivePrefix = {arXiv},
 author = {Nengzheng Jin and Joanna Siebert and Dongfang Li and Qingcai Chen},
 eprint = {2207.05270},
 primaryClass = {cs.CL},
 title = {A Survey on Table Question Answering: Recent Advances},
 year = {2022}
}

@inproceedings{kothyari-etal-2023-crush4sql,
 author = {Kothyari, Mayank  and
Dhingra, Dhruva  and
Sarawagi, Sunita  and
Chakrabarti, Soumen},
 booktitle = {Proc. of EMNLP},
 title = {{CRUSH}4{SQL}: Collective Retrieval Using Schema Hallucination For {T}ext2{SQL}},
 year = {2023}
}

@misc{lei2023tableqakit,
 archivePrefix = {arXiv},
 author = {Fangyu Lei and Tongxu Luo and Pengqi Yang and Weihao Liu and Hanwen Liu and Jiahe Lei and Yiming Huang and Yifan Wei and Shizhu He and Jun Zhao and Kang Liu},
 eprint = {2310.15075},
 primaryClass = {cs.CL},
 title = {TableQAKit: A Comprehensive and Practical Toolkit for Table-based Question Answering},
 year = {2023}
}

@misc{li2023llatrieval,
 archivePrefix = {arXiv},
 author = {Xiaonan Li and Changtai Zhu and Linyang Li and Zhangyue Yin and Tianxiang Sun and Xipeng Qiu},
 eprint = {2311.07838},
 primaryClass = {cs.CL},
 title = {LLatrieval: LLM-Verified Retrieval for Verifiable Generation},
 year = {2023}
}

@misc{li2024using_rerank,
 archivePrefix = {arXiv},
 author = {Zhenwen Li and Tao Xie},
 eprint = {2401.02115},
 primaryClass = {cs.CL},
 title = {Using LLM to select the right SQL Query from candidates},
 year = {2024}
}

@misc{lightman2023verify,
 archivePrefix = {arXiv},
 author = {Hunter Lightman and Vineet Kosaraju and Yura Burda and Harri Edwards and Bowen Baker and Teddy Lee and Jan Leike and John Schulman and Ilya Sutskever and Karl Cobbe},
 eprint = {2305.20050},
 primaryClass = {cs.LG},
 title = {Let's Verify Step by Step},
 year = {2023}
}

@inproceedings{liu-etal-2021-awakening,
 author = {Liu, Qian  and
Yang, Dejian  and
Zhang, Jiahui  and
Guo, Jiaqi  and
Zhou, Bin  and
Lou, Jian-Guang},
 booktitle = {Proc. of ACL Findings},
 title = {Awakening Latent Grounding from Pretrained Language Models for Semantic Parsing},
 year = {2021}
}

@inproceedings{liu2022tapex,
 author = {Qian Liu and Bei Chen and Jiaqi Guo and Morteza Ziyadi and Zeqi Lin and Weizhu Chen and Jian-Guang Lou},
 booktitle = {Proc. of ICLR},
 title = {{TAPEX}: Table Pre-training via Learning a Neural {SQL} Executor},
 year = {2022}
}

@article{LLMSurvey,
 author = {Zhao, Wayne Xin and Zhou, Kun and Li, Junyi and Tang, Tianyi and Wang, Xiaolei and Hou, Yupeng and Min, Yingqian and Zhang, Beichen and Zhang, Junjie and Dong, Zican and Du, Yifan and Yang, Chen and Chen, Yushuo and Chen, Zhipeng and Jiang, Jinhao and Ren, Ruiyang and Li, Yifan and Tang, Xinyu and Liu, Zikang and Liu, Peiyu and Nie, Jian-Yun and Wen, Ji-Rong},
 journal = {arXiv preprint arXiv:2303.18223},
 title = {A Survey of Large Language Models},
 year = {2023}
}

@misc{luo2023wizardcoder,
 archivePrefix = {arXiv},
 author = {Ziyang Luo and Can Xu and Pu Zhao and Qingfeng Sun and Xiubo Geng and Wenxiang Hu and Chongyang Tao and Jing Ma and Qingwei Lin and Daxin Jiang},
 eprint = {2306.08568},
 primaryClass = {cs.CL},
 title = {WizardCoder: Empowering Code Large Language Models with Evol-Instruct},
 year = {2023}
}

@misc{nakano2022webgpt,
 archivePrefix = {arXiv},
 author = {Reiichiro Nakano and Jacob Hilton and Suchir Balaji and Jeff Wu and Long Ouyang and Christina Kim and Christopher Hesse and Shantanu Jain and Vineet Kosaraju and William Saunders and Xu Jiang and Karl Cobbe and Tyna Eloundou and Gretchen Krueger and Kevin Button and Matthew Knight and Benjamin Chess and John Schulman},
 eprint = {2112.09332},
 primaryClass = {cs.CL},
 title = {WebGPT: Browser-assisted question-answering with human feedback},
 year = {2022}
}

@article{nan-etal-2022-fetaqa,
 author = {Nan, Linyong  and
Hsieh, Chiachun  and
Mao, Ziming  and
Lin, Xi Victoria  and
Verma, Neha  and
Zhang, Rui  and
Kry{\'s}ci{\'n}ski, Wojciech  and
Schoelkopf, Hailey  and
Kong, Riley  and
Tang, Xiangru  and
Mutuma, Mutethia  and
Rosand, Ben  and
Trindade, Isabel  and
Bandaru, Renusree  and
Cunningham, Jacob  and
Xiong, Caiming  and
Radev, Dragomir  and
Radev, Dragomir},
 journal = {Transactions of the Association for Computational Linguistics},
 title = {{F}e{T}a{QA}: Free-form Table Question Answering},
 year = {2022}
}

@inproceedings{nan-etal-2023-enhancing,
 author = {Nan, Linyong  and
Zhao, Yilun  and
Zou, Weijin  and
Ri, Narutatsu  and
Tae, Jaesung  and
Zhang, Ellen  and
Cohan, Arman  and
Radev, Dragomir},
 booktitle = {Proc. of EMNLP Findings},
 title = {Enhancing Text-to-{SQL} Capabilities of Large Language Models: A Study on Prompt Design Strategies},
 year = {2023}
}

@misc{nan2023db_agent,
 archivePrefix = {arXiv},
 author = {Linyong Nan and Ellen Zhang and Weijin Zou and Yilun Zhao and Wenfei Zhou and Arman Cohan},
 eprint = {2311.09721},
 primaryClass = {cs.CL},
 title = {On Evaluating the Integration of Reasoning and Action in LLM Agents with Database Question Answering},
 year = {2023}
}

@inproceedings{ni2023lever,
 author = {Ni, Ansong and Iyer, Srini and Radev, Dragomir and Stoyanov, Ves and Yih, Wen-tau and Wang, Sida I and Lin, Xi Victoria},
 booktitle = {Proc. of ICML},
 title = {Lever: Learning to verify language-to-code generation with execution},
 year = {2023}
}

@inproceedings{NIPS2015_pointer_network,
 author = {Vinyals, Oriol and Fortunato, Meire and Jaitly, Navdeep},
 booktitle = {Proc. of NeurIPS},
 title = {Pointer Networks},
 year = {2015}
}

@inproceedings{parikh-etal-2020-totto,
 author = {Parikh, Ankur  and
Wang, Xuezhi  and
Gehrmann, Sebastian  and
Faruqui, Manaal  and
Dhingra, Bhuwan  and
Yang, Diyi  and
Das, Dipanjan},
 booktitle = {Proc. of EMNLP},
 title = {{ToTTo}: A Controlled Table-To-Text Generation Dataset},
 year = {2020}
}

@inproceedings{pasupat-liang-2015-compositional_wikitablequestions,
 author = {Pasupat, Panupong  and
Liang, Percy},
 booktitle = {Proc. of ACL},
 title = {Compositional Semantic Parsing on Semi-Structured Tables},
 year = {2015}
}

@inproceedings{pi-etal-2022-robustness,
 author = {Pi, Xinyu  and
Wang, Bing  and
Gao, Yan  and
Guo, Jiaqi  and
Li, Zhoujun  and
Lou, Jian-Guang},
 booktitle = {Proc. of ACL},
 title = {Towards Robustness of Text-to-{SQL} Models Against Natural and Realistic Adversarial Table Perturbation},
 year = {2022}
}

@inproceedings{pmlr-v206-tabllm,
 author = {Hegselmann, Stefan and Buendia, Alejandro and Lang, Hunter and Agrawal, Monica and Jiang, Xiaoyi and Sontag, David},
 booktitle = {Proc. of AISTATS},
 title = {TabLLM: Few-shot Classification of Tabular Data with Large Language Models},
 year = {2023}
}

@article{pretrain_prompt_survey,
 author = {Liu, Pengfei and Yuan, Weizhe and Fu, Jinlan and Jiang, Zhengbao and Hayashi, Hiroaki and Neubig, Graham},
 journal = {ACM Comput. Surv.},
 title = {Pre-train, Prompt, and Predict: A Systematic Survey of Prompting Methods in Natural Language Processing},
 year = {2023}
}

@inproceedings{pryzant-etal-2023-automaticprompt,
 author = {Pryzant, Reid  and
Iter, Dan  and
Li, Jerry  and
Lee, Yin  and
Zhu, Chenguang  and
Zeng, Michael},
 booktitle = {Proc. of EMNLP},
 title = {Automatic Prompt Optimization with {``}Gradient Descent{''} and Beam Search},
 year = {2023}
}

@misc{qin2022survey_texttosql,
 archivePrefix = {arXiv},
 author = {Bowen Qin and Binyuan Hui and Lihan Wang and Min Yang and Jinyang Li and Binhua Li and Ruiying Geng and Rongyu Cao and Jian Sun and Luo Si and Fei Huang and Yongbin Li},
 eprint = {2208.13629},
 primaryClass = {cs.CL},
 title = {A Survey on Text-to-SQL Parsing: Concepts, Methods, and Future Directions},
 year = {2022}
}

@misc{qin2023tool,
 archivePrefix = {arXiv},
 author = {Yujia Qin and Shengding Hu and Yankai Lin and Weize Chen and Ning Ding and Ganqu Cui and Zheni Zeng and Yufei Huang and Chaojun Xiao and Chi Han and Yi Ren Fung and Yusheng Su and Huadong Wang and Cheng Qian and Runchu Tian and Kunlun Zhu and Shihao Liang and Xingyu Shen and Bokai Xu and Zhen Zhang and Yining Ye and Bowen Li and Ziwei Tang and Jing Yi and Yuzhang Zhu and Zhenning Dai and Lan Yan and Xin Cong and Yaxi Lu and Weilin Zhao and Yuxiang Huang and Junxi Yan and Xu Han and Xian Sun and Dahai Li and Jason Phang and Cheng Yang and Tongshuang Wu and Heng Ji and Zhiyuan Liu and Maosong Sun},
 eprint = {2304.08354},
 primaryClass = {cs.CL},
 title = {Tool Learning with Foundation Models},
 year = {2023}
}

@misc{Radford2018gpt1,
 author = {Alec Radford and Karthik Narasimhan},
 title = {Improving Language Understanding by Generative Pre-Training},
 year = {2018}
}

@inproceedings{resdsql,
 author = {Li, Haoyang and Zhang, Jing and Li, Cuiping and Chen, Hong},
 booktitle = {Proc. of AAAI},
 title = {RESDSQL: decoupling schema linking and skeleton parsing for text-to-SQL},
 year = {2023}
}

@inproceedings{rule_texttosql,
 author = {Mahmud, Tanzim and Azharul Hasan, K. M. and Ahmed, Mahtab and Thwoi Hla Ching Chak},
 booktitle = {2015 2nd International Conference on Electrical Information and Communication Technologies (EICT)},
 title = {A rule based approach for NLP based query processing},
 year = {2015}
}

@inproceedings{saha-etal-2023-murmur,
 author = {Saha, Swarnadeep  and
Yu, Xinyan  and
Bansal, Mohit  and
Pasunuru, Ramakanth  and
Celikyilmaz, Asli},
 booktitle = {Proc. of ACL Findings},
 title = {{MURMUR}: Modular Multi-Step Reasoning for Semi-Structured Data-to-Text Generation},
 year = {2023}
}

@inproceedings{scholak-etal-2021-picard,
 author = {Scholak, Torsten  and
Schucher, Nathan  and
Bahdanau, Dzmitry},
 booktitle = {Proc. of EMNLP},
 title = {{PICARD}: Parsing Incrementally for Constrained Auto-Regressive Decoding from Language Models},
 year = {2021}
}

@article{self-refine,
 author = {Aman Madaan and Niket Tandon and Prakhar Gupta and Skyler Hallinan and Luyu Gao and Sarah Wiegreffe and Uri Alon and Nouha Dziri and Shrimai Prabhumoye and Yiming Yang and Sean Welleck and Bodhisattwa Prasad Majumder and Shashank Gupta and Amir Yazdanbakhsh and Peter Clark},
 journal = {CoRR},
 title = {Self-Refine: Iterative Refinement with Self-Feedback},
 year = {2023}
}

@inproceedings{shao-etal-2023-retrieval-augmented,
 author = {Shao, Zhihong  and
Gong, Yeyun  and
Shen, Yelong  and
Huang, Minlie  and
Duan, Nan  and
Chen, Weizhu},
 booktitle = {Proc. of EMNLP Findings},
 title = {Enhancing Retrieval-Augmented Large Language Models with Iterative Retrieval-Generation Synergy},
 year = {2023}
}

@misc{sui2023tap4llm,
 archivePrefix = {arXiv},
 author = {Yuan Sui and Jiaru Zou and Mengyu Zhou and Xinyi He and Lun Du and Shi Han and Dongmei Zhang},
 eprint = {2312.09039},
 primaryClass = {cs.CL},
 title = {TAP4LLM: Table Provider on Sampling, Augmenting, and Packing Semi-structured Data for Large Language Model Reasoning},
 year = {2023}
}

@inproceedings{sun-etal-2023-sqlprompt,
 author = {Sun, Ruoxi  and
Arik, Sercan  and
Sinha, Rajarishi  and
Nakhost, Hootan  and
Dai, Hanjun  and
Yin, Pengcheng  and
Pfister, Tomas},
 booktitle = {Proc. of EMNLP Findings},
 title = {{SQLP}rompt: In-Context Text-to-{SQL} with Minimal Labeled Data},
 year = {2023}
}

@misc{sun2023test,
 archivePrefix = {arXiv},
 author = {Chenxi Sun and Yaliang Li and Hongyan Li and Shenda Hong},
 eprint = {2308.08241},
 primaryClass = {cs.CL},
 title = {TEST: Text Prototype Aligned Embedding to Activate LLM's Ability for Time Series},
 year = {2023}
}

@inproceedings{tonglet-etal-2023-seer,
 author = {Tonglet, Jonathan  and
Reusens, Manon  and
Borchert, Philipp  and
Baesens, Bart},
 booktitle = {Proc. of EMNLP},
 title = {{SEER} : A Knapsack approach to Exemplar Selection for In-Context {H}ybrid{QA}},
 year = {2023}
}

@article{unisar,
 author = {Dou, Longxu and Gao, Yan and Pan, Mingyang and Wang, Dingzirui and Che, Wanxiang and Lou, Jian-Guang and Zhan, Dechen},
 journal = {International Journal of Machine Learning and Cybernetics},
 title = {UniSAr: a unified structure-aware autoregressive language model for text-to-SQL semantic parsing},
 year = {2023}
}

@inproceedings{wang-etal-2020-rat,
 author = {Wang, Bailin  and
Shin, Richard  and
Liu, Xiaodong  and
Polozov, Oleksandr  and
Richardson, Matthew},
 booktitle = {Proc. of ACL},
 title = {{RAT-SQL}: Relation-Aware Schema Encoding and Linking for Text-to-{SQL} Parsers},
 year = {2020}
}

@misc{wang2023dbcopilot,
 archivePrefix = {arXiv},
 author = {Tianshu Wang and Hongyu Lin and Xianpei Han and Le Sun and Xiaoyang Chen and Hao Wang and Zhenyu Zeng},
 eprint = {2312.03463},
 primaryClass = {cs.CL},
 title = {DBCopilot: Scaling Natural Language Querying to Massive Databases},
 year = {2023}
}

@misc{wang2023macsql,
 archivePrefix = {arXiv},
 author = {Bing Wang and Changyu Ren and Jian Yang and Xinnian Liang and Jiaqi Bai and Qian-Wen Zhang and Zhao Yan and Zhoujun Li},
 eprint = {2312.11242},
 primaryClass = {cs.CL},
 title = {MAC-SQL: Multi-Agent Collaboration for Text-to-SQL},
 year = {2023}
}

@misc{wang2023survey_hybridqa,
 archivePrefix = {arXiv},
 author = {Dingzirui Wang and Longxu Dou and Wanxiang Che},
 eprint = {2212.13465},
 primaryClass = {cs.CL},
 title = {A Survey on Table-and-Text HybridQA: Concepts, Methods, Challenges and Future Directions},
 year = {2023}
}

@inproceedings{wei2022Zero-Shot-Learners,
 author = {Jason Wei and Maarten Bosma and Vincent Zhao and Kelvin Guu and Adams Wei Yu and Brian Lester and Nan Du and Andrew M. Dai and Quoc V Le},
 booktitle = {Proc. of ICLR},
 title = {Finetuned Language Models are Zero-Shot Learners},
 year = {2022}
}

@misc{xi2023agent_survey,
 archivePrefix = {arXiv},
 author = {Zhiheng Xi and Wenxiang Chen and Xin Guo and Wei He and Yiwen Ding and Boyang Hong and Ming Zhang and Junzhe Wang and Senjie Jin and Enyu Zhou and Rui Zheng and Xiaoran Fan and Xiao Wang and Limao Xiong and Yuhao Zhou and Weiran Wang and Changhao Jiang and Yicheng Zou and Xiangyang Liu and Zhangyue Yin and Shihan Dou and Rongxiang Weng and Wensen Cheng and Qi Zhang and Wenjuan Qin and Yongyan Zheng and Xipeng Qiu and Xuanjing Huang and Tao Gui},
 eprint = {2309.07864},
 primaryClass = {cs.AI},
 title = {The Rise and Potential of Large Language Model Based Agents: A Survey},
 year = {2023}
}

@inproceedings{xie-etal-2022-unifiedskg,
 author = {Xie, Tianbao  and
Wu, Chen Henry  and
Shi, Peng  and
Zhong, Ruiqi  and
Scholak, Torsten  and
Yasunaga, Michihiro  and
Wu, Chien-Sheng  and
Zhong, Ming  and
Yin, Pengcheng  and
Wang, Sida I.  and
Zhong, Victor  and
Wang, Bailin  and
Li, Chengzu  and
Boyle, Connor  and
Ni, Ansong  and
Yao, Ziyu  and
Radev, Dragomir  and
Xiong, Caiming  and
Kong, Lingpeng  and
Zhang, Rui  and
Smith, Noah A.  and
Zettlemoyer, Luke  and
Yu, Tao},
 booktitle = {Proc. of EMNLP},
 title = {{U}nified{SKG}: Unifying and Multi-Tasking Structured Knowledge Grounding with Text-to-Text Language Models},
 year = {2022}
}

@inproceedings{xie2023selfevaluation,
 author = {Yuxi Xie and Kenji Kawaguchi and Yiran Zhao and Xu Zhao and Min-Yen Kan and Junxian He and Qizhe Xie},
 booktitle = {Proc. of NeurIPS},
 title = {Self-Evaluation Guided Beam Search for Reasoning},
 year = {2023}
}

@article{xu2017sqlnet,
 author = {Xu, Xiaojun and Liu, Chang and Song, Dawn},
 journal = {arXiv preprint arXiv:1711.04436},
 title = {SQLNet: Generating Structured Queries From Natural Language Without Reinforcement Learning},
 year = {2017}
}

@misc{xu2023wizardlm,
 archivePrefix = {arXiv},
 author = {Can Xu and Qingfeng Sun and Kai Zheng and Xiubo Geng and Pu Zhao and Jiazhan Feng and Chongyang Tao and Daxin Jiang},
 eprint = {2304.12244},
 primaryClass = {cs.CL},
 title = {WizardLM: Empowering Large Language Models to Follow Complex Instructions},
 year = {2023}
}

@misc{xue2024dbgpt,
 archivePrefix = {arXiv},
 author = {Siqiao Xue and Caigao Jiang and Wenhui Shi and Fangyin Cheng and Keting Chen and Hongjun Yang and Zhiping Zhang and Jianshan He and Hongyang Zhang and Ganglin Wei and Wang Zhao and Fan Zhou and Danrui Qi and Hong Yi and Shaodong Liu and Faqiang Chen},
 eprint = {2312.17449},
 primaryClass = {cs.DB},
 title = {DB-GPT: Empowering Database Interactions with Private Large Language Models},
 year = {2024}
}

@misc{yang2023distill,
 archivePrefix = {arXiv},
 author = {Bohao Yang and Chen Tang and Kun Zhao and Chenghao Xiao and Chenghua Lin},
 eprint = {2309.13182},
 primaryClass = {cs.CL},
 title = {Effective Distillation of Table-based Reasoning Ability from LLMs},
 year = {2023}
}

@misc{yang2023optimizers,
 archivePrefix = {arXiv},
 author = {Chengrun Yang and Xuezhi Wang and Yifeng Lu and Hanxiao Liu and Quoc V. Le and Denny Zhou and Xinyun Chen},
 eprint = {2309.03409},
 primaryClass = {cs.LG},
 title = {Large Language Models as Optimizers},
 year = {2023}
}

@misc{yao2023react,
 archivePrefix = {arXiv},
 author = {Shunyu Yao and Jeffrey Zhao and Dian Yu and Nan Du and Izhak Shafran and Karthik Narasimhan and Yuan Cao},
 eprint = {2210.03629},
 primaryClass = {cs.CL},
 title = {ReAct: Synergizing Reasoning and Acting in Language Models},
 year = {2023}
}

@inproceedings{yao2023treeofthoughts,
 author = {Shunyu Yao and Dian Yu and Jeffrey Zhao and Izhak Shafran and Thomas L. Griffiths and Yuan Cao and Karthik R Narasimhan},
 booktitle = {Proc. of NeurIPS},
 title = {Tree of Thoughts: Deliberate Problem Solving with Large Language Models},
 year = {2023}
}

@inproceedings{yin-etal-2020-tabert,
 author = {Yin, Pengcheng  and
Neubig, Graham  and
Yih, Wen-tau  and
Riedel, Sebastian},
 booktitle = {Proc. of ACL},
 title = {{T}a{BERT}: Pretraining for Joint Understanding of Textual and Tabular Data},
 year = {2020}
}

@inproceedings{yu-etal-2018-spider,
 author = {Yu, Tao  and
Zhang, Rui  and
Yang, Kai  and
Yasunaga, Michihiro  and
Wang, Dongxu  and
Li, Zifan  and
Ma, James  and
Li, Irene  and
Yao, Qingning  and
Roman, Shanelle  and
Zhang, Zilin  and
Radev, Dragomir},
 booktitle = {Proc. of EMNLP},
 title = {{S}pider: A Large-Scale Human-Labeled Dataset for Complex and Cross-Domain Semantic Parsing and Text-to-{SQL} Task},
 year = {2018}
}

@inproceedings{yu2021grappa,
 author = {Tao Yu and Chien-Sheng Wu and Xi Victoria Lin and bailin wang and Yi Chern Tan and Xinyi Yang and Dragomir Radev and richard socher and Caiming Xiong},
 booktitle = {Proc. of ICLR},
 title = {Gra{\{}PP{\}}a: Grammar-Augmented Pre-Training for Table Semantic Parsing},
 year = {2021}
}

@inproceedings{yu2023generate_rather_retrieve,
 author = {Wenhao Yu and Dan Iter and Shuohang Wang and Yichong Xu and Mingxuan Ju and Soumya Sanyal and Chenguang Zhu and Michael Zeng and Meng Jiang},
 booktitle = {Proc. of ICLR},
 title = {Generate rather than Retrieve: Large Language Models are Strong Context Generators},
 year = {2023}
}

@misc{zha2023tablegpt,
 archivePrefix = {arXiv},
 author = {Liangyu Zha and Junlin Zhou and Liyao Li and Rui Wang and Qingyi Huang and Saisai Yang and Jing Yuan and Changbao Su and Xiang Li and Aofeng Su and Tao Zhang and Chen Zhou and Kaizhe Shou and Miao Wang and Wufang Zhu and Guoshan Lu and Chao Ye and Yali Ye and Wentao Ye and Yiming Zhang and Xinglong Deng and Jie Xu and Haobo Wang and Gang Chen and Junbo Zhao},
 eprint = {2307.08674},
 primaryClass = {cs.AI},
 title = {TableGPT: Towards Unifying Tables, Nature Language and Commands into One GPT},
 year = {2023}
}

@misc{zhang2023actsql_autocot,
 archivePrefix = {arXiv},
 author = {Hanchong Zhang and Ruisheng Cao and Lu Chen and Hongshen Xu and Kai Yu},
 eprint = {2310.17342},
 primaryClass = {cs.CL},
 title = {ACT-SQL: In-Context Learning for Text-to-SQL with Automatically-Generated Chain-of-Thought},
 year = {2023}
}

@misc{zhang2023beamretrieval,
 archivePrefix = {arXiv},
 author = {Jiahao Zhang and Haiyang Zhang and Dongmei Zhang and Yong Liu and Shen Huang},
 eprint = {2308.08973},
 primaryClass = {cs.CL},
 title = {Beam Retrieval: General End-to-End Retrieval for Multi-Hop Question Answering},
 year = {2023}
}

@misc{zhang2023reactable,
 archivePrefix = {arXiv},
 author = {Yunjia Zhang and Jordan Henkel and Avrilia Floratou and Joyce Cahoon and Shaleen Deep and Jignesh M. Patel},
 eprint = {2310.00815},
 primaryClass = {cs.DB},
 title = {ReAcTable: Enhancing ReAct for Table Question Answering},
 year = {2023}
}

@misc{zhang2023tablellama,
 archivePrefix = {arXiv},
 author = {Tianshu Zhang and Xiang Yue and Yifei Li and Huan Sun},
 eprint = {2311.09206},
 primaryClass = {cs.CL},
 title = {TableLlama: Towards Open Large Generalist Models for Tables},
 year = {2023}
}

@inproceedings{zhao-etal-2022-reastap,
 author = {Zhao, Yilun  and
Nan, Linyong  and
Qi, Zhenting  and
Zhang, Rui  and
Radev, Dragomir},
 booktitle = {Proc. of EMNLP},
 title = {{R}eas{TAP}: Injecting Table Reasoning Skills During Pre-training via Synthetic Reasoning Examples},
 year = {2022}
}

@inproceedings{zhao-etal-2023-parseres,
 author = {Zhao, Bowen  and
Ji, Changkai  and
Zhang, Yuejie  and
He, Wen  and
Wang, Yingwen  and
Wang, Qing  and
Feng, Rui  and
Zhang, Xiaobo},
 booktitle = {Proc. of EMNLP},
 title = {Large Language Models are Complex Table Parsers},
 year = {2023}
}

@inproceedings{zhao-yang-2022-tablefact_plm_lka,
 author = {Zhao, Guangzhen  and
Yang, Peng},
 booktitle = {Proc. of COLING},
 title = {Table-based Fact Verification with Self-labeled Keypoint Alignment},
 year = {2022}
}

@inproceedings{zheng-etal-2023-taco,
 author = {Zheng, Mingyu  and
Yang, Hao  and
Jiang, Wenbin  and
Lin, Zheng  and
Lyu, Yajuan  and
She, Qiaoqiao  and
Wang, Weiping},
 booktitle = {Proc. of EMNLP Findings},
 title = {Chain-of-Thought Reasoning in Tabular Language Models},
 year = {2023}
}

@misc{zheng2023finetunin_survey,
 archivePrefix = {arXiv},
 author = {Hongling Zheng and Li Shen and Anke Tang and Yong Luo and Han Hu and Bo Du and Dacheng Tao},
 eprint = {2310.08184},
 primaryClass = {cs.AI},
 title = {Learn From Model Beyond Fine-Tuning: A Survey},
 year = {2023}
}

@inproceedings{zhong-etal-2023-apel,
 author = {Zhong, Ruiqi  and
Snell, Charlie  and
Klein, Dan  and
Eisner, Jason},
 booktitle = {Proc. of EMNLP},
 title = {Non-Programmers Can Label Programs Indirectly via Active Examples: A Case Study with Text-to-{SQL}},
 year = {2023}
}

@misc{zhong2018seq2sql,
 author = {Victor Zhong and Caiming Xiong and Richard Socher},
 title = {Seq2{SQL}: Generating Structured Queries From Natural Language Using Reinforcement Learning },
 year = {2018}
}


==> old_version/1.introduction.tex <==
% 表格推理任务，显著提升了从大量表格中获取和处理数据的效率，在计算机领域，特别是自然语言处理（Natural Language Processing，NLP）的研究中扮演着重要角色
Table reasoning task, which significantly improves the efficiency of obtaining and processing data from massive amounts of tables, plays an important role in computing, especially in the study of Natural Language Processing (NLP)~\cite{jin2022survey_tableqa}.
% 该任务要求模型在给定一个或多个表格的情况下，按照任务要求，生成相应的结果作为答案（例如：表格问答、表格事实判断）
Given one or more tables, this task requires the model to generate results corresponding to the given question, as required by users (e.g., table QA~\cite{pasupat-liang-2015-compositional_wikitablequestions}, table fact verification~\cite{2019TabFactA}).

% 过去表格推理的研究大致经过了基于规则、基于神经网络以及基于预训练模型（Pre-Trained Language Model）几个阶段
In the past, research in table reasoning has gone through several phases: rule-based~\cite{rule_texttosql,NIPS2015_pointer_network,xu2017sqlnet}, neural network-based~\cite{bogin-etal-2019-representing_gnn,wang-etal-2020-rat}, and pre-trained language model-based~\cite{liu2022tapex,zhao-etal-2022-reastap,unisar}, which we call \textbf{pre-LLM era}.
% 最近的研究表明，大规模语言模型（Large Language Model，LLM）在各个NLP任务上都表现出了引人注目的性能，尤其是，无需大规模数据微调就能迁移到各个任务上的上下文学习能力，极大地降低了标注需求
Recent research~\cite{LLMSurvey} has shown that Large Language Models (LLMs) exhibit compelling performance across NLP tasks, in particular, the ability of in-context learning without large-scale data fine-tuning dramatically reduces annotation requirements, which we call \textbf{LLM era}.
% 考虑到表格推理较高的标注和训练开销，已有许多工作将LLM应用到表格推理任务上，成为了目前的主流方法
Considering the high annotation and training overheads of table reasoning in the pre-LLM era, there has been a lot of work on applying LLMs to table reasoning tasks to reduce the overheads, which has become the current mainstream method.

% 然而，目前缺乏关于LLM表格推理工作的总结分析， leading the improvement is still under exploration，一定程度阻碍了现有研究
However, there is currently a lack of summary analysis on LLM table reasoning works, leading to the improvement of current works is still under exploration, which hinders existing research to a certain extent.
% 而基于PLM的总结分析不适用于LLM，因为一些前大模型时代的主流技不再适用于LLM，其中PLM方法往往采用改变模型结构或设计预训练任务，而LLM方法则更关注在不改变模型的情况下更好地设计prompt或pipeline来提升性能（引LLM survey），导致PLM方法无法直接用于LLM
Besides, the analysis of pre-LLM is not suitable for LLM, because some mainstream techniques in the pre-LLM era, such as changing the model structure and designing pre-training tasks \cite{qin2022survey_texttosql,wang2023survey_hybridqa}, are not suitable for LLM in table reasoning, since LLM methods focus more on designing prompts or pipelines \cite{LLMSurvey}. 
% 因此，我们在本文对现有的基于LLM的表格推理相关工作进行梳理，来促进该领域上的研究
Therefore, this paper summarizes the existing works on table reasoning with LLMs to shed light on future research.
% 在本文中，我们主要讨论三个关于表格推理的topic：1. LLM时代的主流技术; 2. LLM时代带来的提升; 3. LLM时代的未来方向
In detail, we focus on three topics of the table reasoning: \textit{1. the mainstream techniques of the LLM era}; \textit{2. the improvement brought by the LLM}; \textit{3. future directions of the LLM era}.

% 关于第一个topic，我们首先在第2节介绍了背景，作为我们后续分析的基础。
Regarding the first topic, we introduce the table reasoning task background in $\S$\ref{sec:background}, as a basis for subsequent analyses. 
% 为了帮助研究者更好地适应LLM时代的表格推理研究，我们介绍了LLM时代的主流技术
To help researchers better adapt to the LLM era of table reasoning, we present the main techniques of the LLM era in $\S$\ref{sec:analysis}

About the second topic, we categorize and summarize how the existing methods improve the table reasoning performance of LLMs following the mainstream techniques in $\S$\ref{sec:category} and $\S$\ref{sec:methodology}\footnote{We summarize the performance of the current methods on each benchmarks in \url{https://github.com/zhxlia/Awesome-TabelReasoning-LLM-Survey}.} to better understand how to utilize the techniques in LLM era.
We then analyze the key insights behind the improvement brought by LLM.

% 关于第三个topic，我们在第5节讨论了未来潜在的方向。
Considering the third topic, we discuss potential future directions for improvement in $\S$\ref{sec:future}.
% 为了促进表格推理方法更好地应用于现实场景，我们分析了结合现实场景需求并据此提出了可能的改进方向。
To promote the table reasoning method to be better applied to actual scenarios, we analyze the needs of actual scenarios and propose possible improvement directions accordingly.


\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\textwidth]{tex/fig/def.pdf}
    \caption{The summary of the table reasoning task.}
    \label{fig:intro}
\end{figure*}













% The previous techniques of table reasoning, such as changing the model structure, and designing pre-training tasks, can not be directly used in LLM, while the mainstream techniques of LLM focus more on better designing prompts or pipelines to improve performance \cite{LLMSurvey}.
% 然而，there is a need to 对现有表格推理with LLM工作的总结分析，因为现有很多用LLM解决表格推理的工作，但仍然缺乏对这种工作的总结与分析
% However, there are many existing works using LLM to solve table reasoning, but there is still a lack of summary and analysis of these works.
% However, despite many existing works, there is still a lack of summary and analysis of table reasoning works with LLMs.
% 而由于基于PLM的总结更关注PLM的表格推理方法，而PLM方法往往单独用一个模型来解决一个挑战，而由于LLM更大的模型规模以及多样的训练任务，一个LLM可以解决所有挑战，导致PLM方法无法直接用于LLM，导致现有关于表格推理工作的可改进之处仍有待研究，一定程度阻碍了现有研究
% Since the summary and analysis of PLMs~\cite{qin2022survey_texttosql,wang2023survey_hybridqa} pay more attention to the methods of table reasoning, which often uses a single model to solve a challenge, compared with LLM methods solving all challenges with one model due to its larger model scale and more diverse training tasks, resulting in PLM methods cannot be directly used in LLM and improvements in LLM table reasoning work still needs to be studied, which hinders existing research to a certain extent.
% 而由于基于PLM的总结更关注PLM的表格推理方法，导致PLM时代的总结分析无法直接适用于LLM，导致现有关于表格推理工作的可改进之处仍有待研究，一定程度阻碍了现有研究
% Since the summary and analysis of PLMs~\cite{qin2022survey_texttosql,jin2022survey_tableqa,wang2023survey_hybridqa} pay more attention to the PLM methods of table reasoning which cannot be directly applied to LLMs because of the different structures and model scales of PLMs and LLMs, resulting in the improvement of existing table reasoning work with LLMs is still under discovery, which hinders research to a certain extent.

==> old_version/3.analysis.tex <==
% What are the Main Techniques in the LLM Era
% 研究者对pre-LLM方法和LLM方法在改进思路上有很大不同
There are significant differences between the model ability of the pre-LLM era and the LLM era, leading to the difference in the mainstream techniques \cite{LLMSurvey}.
% 为了帮助研究者更好地把基于pre-LLM的研究过渡到基于LLM的研究，在这一节，我们将从可以从pre-LLM能够继承的改进（\S），和在LLM时代独有的改进（\S）两方面，讨论LLM方法未来的improvement direction
To help researchers better transition from pre-LLM research to LLM-based research, in this section, we discuss the mainstream techniques of the LLM methods from two aspects, the techniques following pre-LLM era (\S\ref{subsec:Improvement Directions Following pre-LLM Era}), and techniques unique to LLM era (\S\ref{subsec:Improvement Directions of LLM era}).

\subsection{Mainstream Techniques Following pre-LLM Era}
% What mainstream techniques in the pre-LLM era can be used in the LLM era
    \label{subsec:Improvement Directions Following pre-LLM Era}
    % 尽管LLM带来了很大的研究上的转变，但很多pre-LLM的技术依然可以沿用到LLM上
    Despite the considerable change in research brought about by LLMs, many pre-LLM techniques can still be applied to LLM.
    % 因此在这一节，我们介绍从pre-LLM沿用的研究思路
    Therefore, we introduce the LLM mainstream techniques following the pre-LLM era in this subsection.

    \paragraph{Fine-Tuning}
        % 微调，指 a transfer learning technique for using the knowledge of pre-trained neural networks to solve new, relevant tasks
        Fine-tuning is a method of transfer learning that utilizes the expertise of PLMs to address new, related tasks \cite{zheng2023finetunin_survey}.
        % 因为微调以较小的训练开销在广泛的数据集上证明了其对特定任务提升性能的有效性，所以是前大模型时代研究者常用的方法之一
        Because fine-tuning proves its effectiveness in improving performance with relatively small training overhead on a wide range of benchmarks, it is one of the methods commonly used by researchers in the pre-LLM era \cite{Radford2018gpt1}.
        % 而在LLM时代，依然可以通过微调增强LLM的性能
        In the LLM era, LLM performance can still be enhanced through fine-tuning.
        % 虽然部分LLM在不同任务上均表现出了较强的能力，但也有一些LLM解决某些复杂任务，如表格推理任务，的能力较弱 
        Although some LLMs have shown strong abilities in different tasks, some LLMs are weak in solving certain complex tasks, such as table reasoning tasks \cite{zhang2023tablellama}.
        % 为了提升这些LLM在这些复杂任务上的能力，研究者通过构建训练数据对LLM进行微调
        % To improve the capabilities of these LLMs on complex tasks, researchers construct training data and fine-tune the LLMs.
    
    \paragraph{Result Ensemble}
        % 前大模型时代研究者通过集成方法，指融合模型针对同一问题的多个结果，提升模型性能
        In the pre-LLM era, researchers use ensemble methods to improve model performance by voting from multiple results for the same question \cite{ensemble_study}.
        % 考虑到不同模型在面对同一问题时输出结果可能不同，同一模型在输入发生微小变化时，输出的结果也可能发生变化的情况，这种不一致意味着模型无法稳定地生成正确结果 
        Considering that different models could output distinct results when facing the same input and the output of the same model could also change when the input changes slightly, the inconsistency means that the model cannot consistently produce correct results.
        % 为了解决这一问题，研究者采用集成方法，旨在从众多结果中得到正确结果
        To solve this problem, researchers use the ensemble method which enhances the consistency by voting the correct result from multiple candidate results.
        % 因为ensemble只对结果进行处理，所以该方法不受限于模型，而LLM也面临同样的不一致问题，因此研究者同样采用集成方法来提升模型性能
        The ensemble methods can also be used in LLM, since: 1. the ensemble methods only process the results, which are not limited to the model, and 2. LLM also faces the inconsistency problem \cite{ni2023lever}.
    
\subsection{Mainstream Techniques unique to LLM era}
% What mainstream techniques are unique to the LLM era
    \label{subsec:Improvement Directions of LLM era}
    % 在LLM时代，除了Following pre-LLM Era的改进方向，还有独属于LLM的改进方向，由于LLM的涌现现象
    In the LLM era, in addition to the mainstream techniques following the pre-LLM Era, there are also techniques unique to LLM due to the emergence phenomenon \cite{LLMSurvey}.
    % 因为涌现能力为LLM方法带来了新的改进方向，因此在这一节我们介绍这些不同于前大模型时代的改进方向
    Because emergent abilities bring novel mainstream techniques to the LLM methods, we introduce these techniques in this subsection.
    \paragraph{In-Context Learning}
        % In-Context Learning指语言模型根据提供的自然语言指令和/或多项任务演示，可以通过完成输入指令的预期输出，而不需要额外的训练或梯度更新
        The in-context learning ability means that the model can generate the expected answer based on the provided natural language instruction and multiple demonstrations, which are called prompts, without requiring additional training or gradient updates \cite{gpt3}.
        % 由于上下文学习的性能受prompt严重影响，因此可以通过设计prompt，包括指令和示例，来提升模型性能，而无需微调
        Since the performance of in-context learning can be significantly affected by prompts, LLM performance can be improved by simply designing input prompts.
        % 比如在表格推理任务上，研究者可以通过利用LLM的上下文学习能力设计合适的表格指令和示例，来提升模型的表格推理性能
        % For example, in the table reasoning tasks, researchers can utilize the in-context learning capabilities of LLM to design appropriate table instructions and examples to improve the model performance of table reasoning.

    \paragraph{Instruction Following}
        % Instruction Following指LLM即使在未见过的任务上，依据指令描述也可以表现得很好
        The instruction following means that LLM can solve the tasks that are unseen in the pre-training phase according to the instruction description \cite{wei2022Zero-Shot-Learners}.
        % 由于LLM具有这种很好的泛化性，因此相比较pre-LLM，研究者可以根据需要将LLM用于更多样的任务上
        Because LLM has such superior generalization, researchers can use LLM for more diverse tasks as needed compared to pre-LLM.
        % 这也为解决复杂任务带来了便利，因为将任务分解可以降低求解难度，研究者可以充分利用LLM的指令跟随能力来解决每个分解的任务而无需为每个分解任务微调
        % This also brings convenience to solving complex tasks by decomposing the task can reduce the difficulty of solving the problem, and researchers can make full use of the instruction following ability to solve each decomposed task without fine-tuning for each decomposed task.

    \paragraph{Step-by-Step Reasoning}
        % Step-by-Step Reasoning指LLM可以通过利用涉及中间推理步骤的提示机制来解决复杂推理，以得出最终答案
        The ability for step-by-step reasoning indicates that solving complex reasoning tasks by employing prompt mechanisms that incorporate intermediate reasoning stages \cite{cot}.
        % 因为这种能力可以显著提升LLM执行复杂推理的能力，所以相比较pre-LLM，LLM在复杂推理任务上的性能也得到了进一步的提升
        The step-by-step reasoning significantly improves the complex reasoning performance by prompting the LLM to reason in multi-steps, compared with pre-LLM \cite{chu2023cot_survey}.
        % 因此，在LLM时代，研究者可以通过设计提示引导模型对复杂的推理任务进行一步步的推理，比如，在表格推理任务上，用LLM一步步推理显著提升了模型性能
        % Therefore, in the LLM era, researchers design prompts to guide the model to perform step-by-step reasoning on complex reasoning tasks.
        


==> old_version/4.category.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{tex//fig/cat.pdf}
    \caption{The illustration of the five method categories: supervised fine-tuning, modular decomposition, prompt design, tool learning, and results ensemble.}
    \label{fig:category}
\end{figure*}

% 为了帮助研究者们更深入地了解从何种角度使用LLM的主流技术去提升模型的表格推理能力，我们将现有基于LLM的表格推理相关研究在方法的角度分为5类，分别为。。。
To help researchers gain an understanding of the perspectives on how to utilize the mainstream techniques of the LLM era to enhance table reasoning, we categorize the existing research into five categories from a view of methodology, 
respectively supervised fine-tuning\S\ref{subsec:category_sft}, modular decomposition\S\ref{subsec:category_md}, prompt design\S\ref{subsec:category_pd}, tool learning\S\ref{subsec:category_tl}, and results ensemble\S\ref{subsec:category_re}. 
The illustration of the five method categories is shown in Figure~\ref{fig:category}.
% 我们将在本节介绍分类的定义、原因，以及和PLM时代的变化，为了帮助研究者更好基于LLM的主流技术适应表格推理
For each category, we introduce its definition, the reason for its categorization criteria, and the changes compared with methods in the pre-LLM era to help researchers better adapt to table reasoning following the mainstream techniques of the LLM era.

\subsection{Supervised Fine-Tuning}
% supervised fine-tuning can enhance the table reasoning capability
    \label{subsec:category_sft}
    % 有监督微调是指用有标注数据微调LLM，从而增强LLM的表格推理能力，因为部分大模型在表格推理方面的能力较弱，相比较其它能力较强的LLM。
    Considering the \textbf{fine-tuning} mainstream technique, supervised fine-tuning refers to fine-tuning the LLM with annotated data to enhance the table reasoning capabilities since some open-source models are weak in solving table tasks \cite{zhang2023tablellama} compared to other LLMs with stronger capabilities which do not need supervised fine-tuning.
    % 现有的研究结果表明，部分开源大模型解决表格相关任务的能力较弱，为了提升模型的表格推理能力，研究者们提出采用有监督微调的方法来解决这一问题。
    % To solve the problem, researchers have proposed using supervised fine-tuning methods, improving the table reasoning capabilities of models.  
    % 在PLM时代，研究者会用单一任务的数据微调模型，而现在，人们会用多个任务的混合数据微调LLM，since LLM可以泛化到多种任务上，并且可以保持在每个任务上的性能
    In the pre-LLM era, researchers use single-task data to fine-tune models, but currently, people use data from diverse tasks to fine-tune LLM, since LLM can generalize to a variety of tasks.
    However, the new challenges researchers face are how to obtain diverse data from different tasks effectively.
    
    % 也会对模型有监督微调，但与LLM时代不同，研究者只能期待提升模型在某一类表格推理任务上的性能，受限于预训练模型的能力，无法通过微调提升模型在所有表格推理任务上的泛化能力。
    % In the PLM era, researchers also take supervised fine-tuning~\cite{wang-etal-2020-rat}.
    % However, due to the limited ability of the pre-trained models, researchers can only improve the performance on one task but not improve the model's generalization to all table reasoning tasks through fine-tuning, just like LLMs.
    
\subsection{Modular Decomposition}
    \label{subsec:category_md}
    % 模块化分解指将复杂任务显式地分解为多个子任务，来完成表格推理任务。
    Modular decomposition is the explicit decomposition of a complex table reasoning task into multiple sub-tasks, which requires the \textit{instruction following} ability.
    % 研究者发现将任务分解为简单的子任务后，完成各个子任务比完成整个复杂任务更为容易，可以提升LLM在复杂任务上的性能，所以希望通过合理分解复杂表格推理任务来提升模型性能。
    The researchers find that it is easier to complete individual decomposed sub-tasks than to complete the whole complex task \cite{din-sql}, thereby improving the performance of LLM on complex tasks, proving the effectiveness of modular decomposition.
    
    % 在用PLM解决表格推理任务时，人们也会通过将任务模块化分解为简单子任务来降低整体任务难度，但针对每一个子任务都需要额外的训练数据单独训练一个模型来解决，而LLM可以很好地利用其上下文学习能力及泛化性，不再需要对每一个表格类子任务专门训练。
    When solving table reasoning tasks with pre-LLMs, people also decompose the task into sub-tasks to reduce the difficulty of the task, however, each sub-task requires a separate model to solve it \cite{unisar}. 
    % 因为LLM具有复杂的模型结构和多样化的训练数据，可以在多个任务上保持很好的性能，所以不再需要为每个模块单独训练一个模型来完成子任务
    In contrast, because LLM has a complex model structure and diverse training data, it can maintain good performance on multiple tasks, so it is no longer necessary to train a separate model for each module to complete each sub-task.
    
\subsection{Prompt Engineering}
    \label{subsec:category_pd}
    % prompt设计指LLM在不用微调的情况下，通过更好地设计prompt，包括instruction和demonstration来增强表格推理能力。
    Prompt engineering means activating the \textit{in-context learning} and \textit{step-by-step reasoning} abilities of LLMs for table reasoning by designing prompts, which include instructions and demonstrations, without fine-tuning.
    Since the performance of LLM is heavily dependent on the input prompt, how to design a better prompt to improve the table reasoning ability has become a problem that needs to be investigated \cite{icl-survey}. 
    
    % prompt在没有对模型进行微调的情况下对PLM的性能影响没有对LLM的影响显著，因为PLM用于预训练的任务与表格推理任务差距较大，所以在PLM时代研究者很少通过设计prompt来提升模型的表格推理性能
    On the contrary, the prompt impact on the table reasoning performance of pre-LLMs is not significant without using the prompt to fine-tune, since there is a big gap between the pre-training tasks and table reasoning tasks \cite{pretrain_prompt_survey,yin-etal-2020-tabert}.
    % 但如何根据不同的任务挑选或生成prompt成为了新的挑战
    However, in the LLM era, how to automatically select or generate better instructions and demonstrations according to different questions has become a new challenge.
    
    % 上下文学习是指LLM在不用微调的情况下，通过设计prompt来增强表格推理能力。
    % In-context learning refers to enhancing the ability of LLMs to table reasoning by designing the prompt without fine-tuning.
    % 研究者们认为部分LLM无需微调就已经具备表格推理能力，可以通过In-Context Learning解锁这种能力。
    % The previous research shows that some LLMs are already capable of table reasoning without fine-tuning, which can be enhanced through in-context learning \cite{chen-2023-few}.
    % 但由于LLM的表现性能严重依赖于输入的上下文，如何通过上下文学习更好地激发模型的表格推理能力成为一个需要研究的问题。
    % However, since the performance of in-context learning is heavily dependent on the input prompt, how to design a better prompt to improve the model's table reasoning ability through in-context learning has become a problem that needs to be investigated \cite{icl-survey}.
    % LLM的上下文学习能力很好地缓解了PLM对每个任务都需要大量训练的问题，但也带来了新的挑战。
    % The in-context learning capabilities, which the PLMs do not have, can mitigate the previous need for extensive training for every task, but they also present new challenges.
    % 由于人们尚不能探明LLM上下文学习能力的机理，所以只能从上下文学习带来表格推理性能提升的角度试图探索不同的prompt对不同模型的影响。
    % Since the mechanism of in-context learning is still under discovery, one can try to explore the effect of different prompts and design inputs only in terms of the changed performance of table reasoning.
    
\subsection{Tool Learning}
    \label{subsec:category_tl}
    % 工具学习指的是大型语言模型学习和使用各种外部工具来增强其处理和解决表格推理问题的能力
    Tool learning refers to employing the \textit{instruction following} ability of LLMs to make and use various external tools to enhance their ability to handle and solve table reasoning problems \cite{qin2023tool}.
    % 研究者在将复杂表格推理任务分解后，发现LLM并不适用于求解所有子任务，在诸如检索、数值计算等的任务上LLM落后于现有工具或方法，造成总体性能不佳。
    % 所以研究者们开始关注工具学习，具体为如何令LLM合作工具更好地完成表格推理任务,何时使用工具，使用何种工具，以及如何使用工具成为了新的挑战。
    Faced with the decomposed sub-tasks of table reasoning, LLM, despite maintaining acceptable performance on most of the sub-tasks, is not suitable for solving all sub-tasks(e.g, retrieval, numerical reasoning), resulting in poor overall performance \cite{cao-etal-2023-api}, so researchers focus on solving some sub-tasks with tools, however, when to use tools, what tools to use, and how to use them becomes a new challenge in the table reasoning process.
    % PLM并不具有使用工具的能力
    Compared with LLMs, pre-LLMs cannot use diverse tools due to the limitations of traditional supervised learning and reinforcement learning's ineffectiveness in complex decision spaces \cite{qin2023tool}.
    
\subsection{Results Ensemble}
    \label{subsec:category_re}
    % 结果集成指通过集成LLM生成的多个结果提升模型的表格推理能力
    Inspired by the \textit{result ensemble} mainstream technique, LLM can improve table reasoning ability by the method of ensemble faced with multiple results generated by LLM.
    % 研究发现LLM在输入发生微小变化时（例如：随机数种子、问题中的无意义词），保持生成正确结果的能力较为欠缺，即缺少鲁棒性，导致模型性能衰退。
    LLM is less capable of generating correct results when the input changes slightly (e.g., random number seeds, meaningless words in questions), which is the lack of robustness, leading to model performance degradation \cite{ni2023lever}.

    % 为了提升模型的鲁棒性，PLM时代人们会采用对抗训练或改变输入的方法，而在LLM时代人们目前采用了对生成结果的集成的方法。
    In the pre-LLM era, researchers take the method of modifying the model input \cite{gan-etal-2021-robustness_Text-to-SQL} or adversarial training \cite{pi-etal-2022-robustness}, while in the LLM era, people enhance the robustness of table reasoning by results ensemble, which only processes the results and does not include additional training.
    % 然而，如何在没有正确答案的情况下在多个结果中选择最正确的是现在研究者面对的挑战
    However, how to obtain multiple results and how to select the correct one without a gold answer is a challenging problem.
    
    % 鲁棒性是指LLM在输出发生微小变化时，依然能保持生成正确结果的能力（例如：随机数种子、问题中的无意义词）。
    % Robustness is the improved ability of the LLM to maintain correct results despite small changes in the input (e.g., random number seeds, nonsense words in a problem).
    % 经过研究发现LLM在生成答案时缺少鲁棒性会导致模型性能衰退。
    % It is found that the lack of robustness of LLM in generating answers leads to the degradation of model performance~\cite{ni2023lever}.
    
    % 提升模型鲁棒性的挑战在PLM时代就已经存在，之前人们普遍通过额外训练来提升PLM在表格推理任务上的鲁棒性[33]，但LLM时代人们目前只是通过对生成结果的处理来提升表格推理结果的鲁棒性。
    % The challenge of improving model robustness in the table reasoning task has existed in the PLM era, where it was common to improve the robustness through additional training~\cite{pi-etal-2022-robustness}. However, in the LLM era people are currently only improving the robustness of table reasoning results through processing generated multiple results.
    % 对结果集成的方法在PLM时代就已经存在

==> old_version/5.methodology.tex <==
\renewcommand{\dblfloatpagefraction}{.9}
\begin{figure*}
    \tiny
    \resizebox{\textwidth}{!}{
        \input{tex/fig/mind_mapping}
    }
    \caption{
        The Summary of Table Reasoning Methods.
    }
    \label{fig:summary}
\end{figure*}

% 为了读者更好地了解现有基于LLM的表格推理任务的研究进展，在本节，我们将详细介绍各自类别下研究者们解决表格推理任务的具体做法，并分析现有工作的研究趋势。
To better understand the existing research progress on how to enhance table reasoning in the LLM era, in this section, we list the specific methods under the five categories in \S\ref{sec:category} and analyze the research trend of current works.
The summary of table reasoning methods under the five categories is shown in Figure~\ref{fig:summary}.

\subsection{Supervised Fine-Tuning}
\label{subsec:supervised fine-tuning}
    % 现有的LLM表格推理的有监督微调工作分为两类：基于已有标注数据集的微调，以及从LLM中蒸馏数据进行微调。
    Existing work on supervised fine-tuning of LLM table reasoning falls into two types: 
    \textit{1}. based on \textbf{pre-existing or manually labeled data}, and 
    \textit{2}. based on \textbf{distilled data} generated by LLMs.
    % 为了让模型更好地完成表格推理任务，TabLLM和TableGPT分别通过挑选少量数据和构造指令数据集微调LLM
    About works on pre-existing or manually labeled data, to better complete table reasoning tasks, TabLLM~\cite{pmlr-v206-tabllm} and TableGPT~\cite{zha2023tablegpt} fine-tune LLMs by selecting labeled data and constructing instruction datasets respectively.
    % **TableLlama**考虑到前人工作只支持特定类型的表格和任务，或者模型微调只能学习到进行预定义的表格操作，因此从广泛使用的数据集中选择具有代表性的表格任务构建了TableInstruct数据集，并在此上微调LLM很好地提升了模型泛化性。
    Considering the lack of generalization of previous work, TableLlama~\cite{zhang2023tablellama} constructs the training data by selecting representative table task datasets.
    % APEL注意到模型需要标注数据训练，尤其是代码类数据，专家标注数据的代价太高，而直接让非专家标注者选择正确的程序又太具挑战，因此提出根据schema生成数据库令信息增益最大，令non-programmers根据问题、数据库和SQL执行结果来判断SQL的正确性，以此获得标注数据。
    Noting that annotating SQL data is too challenging, APEL~\cite{zhong-etal-2023-apel} proposes a method to annotate SQL, which generates the database according to schema and judges SQL correctness based on execution results.
    % TaCo观察到表格模型缺乏CoT能力，而CoT可以提升表格推理能力，所以提出利用有标注数据集微调，先输入表格和问题，微调TaLM生成中间推理步骤，再输入表格、问题和中间推理步骤，微调TaLM生成最终答案。
    % TaCo~\cite{zheng-etal-2023-taco} observes that pre-trained tabular language models(TaLMs) lack the CoT capability which enhances table reasoning, so utilizes the annotated inference steps to fine-tune TaLM.
    
    % 而关于从LLM中蒸馏数据的工作，**Distill**观察到开源小模型在复杂推理的table-to-text任务上的性能落后于LLM，于是使用LLM作为教师模型蒸馏CoT推理和表格描述，并用蒸馏数据微调开源模型，有效地将表格推理能力转移到较小的模型上。
    As for the work on distilled data, \cite{yang2023distill} observes that the performance of the open-source model lagged behind that of LLM on table-to-text tasks, so uses LLM as a teacher model to distill CoT reasoning and table descriptions, and fine-tuned the open-source model.
    % 而**HELLaMA**关注到部分通用模型缺乏根据输入在表格中定位依据的能力，因此通过使用其他LLM根据表格描述预测描述在表格中的位置来获得训练数据微调开源模型。
    And HELLaMA~\cite{bian2023hellama} is concerned that some models could not locate the evidence based on the inputs, therefore it obtains training data to predict where the labeled description would be located by using other LLMs, and then fine-tune models.
    
    % 基于已有数据，或者蒸馏数据体现了LLM时代研究者获取训练数据的两种思路
    % 已有数据集的质量普遍偏高，但领域、种类、难度等较为有限；而蒸馏LLM获得的数据限制较小，但面临需要过滤低质量数据的问题。
    Based on pre-existing or manually labeled data, and distilled data embody the two thoughts to obtain training data in the LLM era.
    Pre-existing datasets are generally of high quality, but more limited in domain, task, and difficulty; whereas distilled data is less restrictive data but faces the problem of needing to filter low-quality data.
    
\subsection{Modular Decomposition}
\label{subsec:modular decomposition}
    % 现有关于模块化分解的研究可以分成两类：一种是在in-domain设置下研究表格推理任务，另一种则是在open-domain设置下
    Existing research with the table reasoning method of modular decomposition can be divided into two directions: 
    \textit{1}. in the \textbf{in-domain} setting, and
    \textit{2}. in the \textbf{open-domain} setting.
    % **DATER**和**DIN-SQL**都注意到将复杂问题分解为简单子问题可以有效促进大模型多步推理，因此两篇文章分别针对表格推理任务，以及单独的text-to-SQL任务设计了不同的流水线方法将复杂推理任务分解来降低模型推理难度。
    About the in-domain works, both DATER~\cite{dater} and DIN-SQL~\cite{din-sql} note that decomposing table reasoning can effectively facilitate multi-step inference, thus they design pipelines for the table reasoning task to reduce the difficulty of inference.
    % **TableQAKit**发现TableQA 任务面临着有巨大差异的数据和任务形式，阻碍了研究的便利性。因此提出了TableQAKit，将TableQA的任务框架分成了配置模块、统一数据形式模块、使用模型模块，以及评估模块,能够支持几乎所有TableQA场景。
    TableQAKit~\cite{lei2023tableqakit} finds that Table QA tasks face different data and task forms, hindering the ease of research, so divide the Table QA task into a configuration module, a data module, a model module, and an evaluation module.
    
    % **CRUSH4SQL**和**OpenTab**则关注到开放域的表格推理任务，通过将任务分解为先检索问题相关表格，再用LLM推理的过程，缓解了大量无关信息的输入给模型带来推理难度增加的问题。
    Regarding the open-domain works, CRUSH4SQL~\cite{kothyari-etal-2023-crush4sql}, OpenTab~\cite{anonymous2023opentab}, and DB-GPT~\cite{xue2024dbgpt} decompose the task into retrieving and reasoning to alleviate the problem of increased difficulty caused by irrelevant information.
    % DBCopilot也关注到开放域的text-to-SQL任务，但不同于检索方法会因问题表示的多样性而与表格数据不匹配导致性能不佳，因此将任务分解为，先使用graph-based constrained decoding algorithm，根据问题预测相关的数据库和表格，再根据生成的schema进行推理生成SQL
    DBCopilot~\cite{wang2023dbcopilot} notices retrieval could suffer from the diverse expressions and vocabulary mismatch, so the task is decomposed into, firstly generating the question-relevant schema instead of retrieving and then reasoning.
    % MAC-SQL发现text-to-SQL任务中，有限的上下文窗口长度阻碍了模型处理大的数据库和表格，并且对复杂查询，single-pass生成SQL会产生错误，生成的SQL也缺乏验证，因此将任务模块化分解为：Selector选择问题相关的表和列，Decomposer用CoT将复杂问题分解为子问题，Refiner迭代检测句法正确性、执行可行性和执行结果非空，并修改
    MAC-SQL~\cite{wang2023macsql} finds that the limited context window, single-pass generation, and the lack of verification result in poor performance, so the task is modularly decomposed into three modules to solve the problems.
    % as follows: the Selector selects the tables and columns, the Decomposer breaks down the question using CoT prompt, and the Refiner iteratively detects and modifies errors.

    % 可以发现，无论是在in-domain设置下还是在open-domain设置下，研究者都事先将任务分解为差异较大的模块，模型按照研究者规定的分解逐步完成每个表格推理的子任务
    % 与in-domain的工作相比，open-domain设置下研究者需要额外关注如何处理海量的表格数据，分解的子任务中会有从大量表格中获得问题相关的表格
    Whether in the in-domain setting or the open-domain setting, the researchers decompose the task into significantly different sub-tasks in advance, and the LLM gradually completes each sub-task according to the decomposition.
    However, compared with in-domain works, open-domain works need to pay extra attention to how to deal with massive table data. Among the decomposed sub-tasks, there exists the sub-task about how to obtain tables related to the question from a large number of tables.
    
\subsection{Prompt Engineering}
\label{subsec:in-context learning}
    The existing table reasoning works of LLM prompt engineering follow two main directions: 
    \textit{1}. prompting the LLM \textbf{single-step} reasoning, and 
    \textit{2}. prompting the LLM \textbf{multi-step} reasoning.
    % 关于直接设计prompt的相关工作，**few(1)-shot**工作最先探索并证明了LLM具有上下文学习的表格推理能力。
    Regarding the prompt engineering for single-step reasoning, \cite{chen-2023-few} is the first to explore and demonstrate that LLM can reason about tables with in-context learning.
    % **ODIS**观察到前人工作在上下文学习时不提供示例，或只提供领域外的示例但研究表明，领域内示例可以显著提高LLM性能，因此提出基于SQL相似度合成领域内SQL，再用LLM生成对应问题作为领域内示例。
    ODIS~\cite{chang-fosler-lussier-2023-selective_odis} observes that in-domain demonstrations can improve performance, so it synthesizes in-domain SQL based on SQL similarity.
    % DAIL-SQL、SEER和Enhancing为了解决上下文学习中的示例选择问题，分别基于masked question similarity、inference chain和SQL similarity选择示例
    To address the challenge of demonstration selection, DAIL-SQL~\cite{gao2023dail}, SEER~\cite{tonglet-etal-2023-seer}, and \cite{nan-etal-2023-enhancing} select demonstrations based on masked question similarity, inference chain, and SQL similarity respectively.
    % **DAIL-SQL**为了系统探索高效prompt工程，提出了基于掩码后问题的相似度选择示例，并且省略其数据库模式以减少输入长度。
    % To explore efficient prompt engineering, DAIL-SQL~\cite{gao2023dail} proposes masked question similarity selection for examples and omits its schema to reduce the input length.
    % 而**SEER**为了解决HybridQA任务在上下文学习中示例选择的挑战，尤其是用户问题和示例中推理路径的相关性小的问题，根据问题向量之间的相似度，以及分类器预测的问题的推理链，从数据中选择示例。
    % To address the challenge of example selection, SEER~\cite{tonglet-etal-2023-seer} selects the examples based on question similarity and the inference chain predicted by classifiers.
    % Enhancing发现，LLM的性能受示例prompt的影响，为了探索text-to-SQL任务中的各种提示策略，提出根据与zero-sho生成的SQL的相似度以及示例的多样性从示例池中选择示例，并且线性化DB时增广列的定义和Entity-Relationship summary
    % \cite{nan-etal-2023-enhancing}, to explore various prompting strategies, selects demonstrations based on SQL similarity and diversity, and linearizes the database with augmentation.
    % Parsers发现前人工作没有关注到复杂表格上的table QA任务，为了更好地解析复杂表格结构，提出重构表格，将表格中的cell解码为五元组.
    To better parse complex tables, \cite{zhao-etal-2023-parseres} proposes to decode the table cells as a tuple which contains rich information.
    % TAP4LLM注意到表格推理任务中，因表格可能超过模型限制的长度、噪音、以及包含模糊信息或专业术语，很难直接作为prompt输入。因此TAP4LLM首先根据问题将表格分解为子表，再结合结合额外知识、元数据等增广原始表格，并且合理平衡表格数据和增广数据的比例。 exceed the length of the model limitation,
    TAP4LLM~\cite{sui2023tap4llm} notices tables could contain noise and ambiguous information, therefore, it decomposes the table with augmentation.
    % Auto-CoT发现，text-to-SQL任务中现有CoT方法需要耗费大量时间和资源在example的选择和CoT标注上，因此提出随机选择静态examples，根据问题相似度选择动态example，利用规则方法schema linking，自动生成example的CoT prompt
    Auto-CoT~\cite{zhang2023actsql_autocot} finds that the existing CoT annotation consumes resources, so uses the rule-based method of schema linking to generate CoT prompts.
    
    % 关于通过prompt多步推理的工作，值得注意的是，与模块化分解,which研究者将任务分解为差别较大的子任务，Prompt LLM多步推理则需要LLM自己将问题分解为多个子问题分步求解
    The prompt engineering for multi-step reasoning, which requires the LLM to decompose the question into multiple sub-questions, is different from modular decomposition, in which researchers break down tasks into widely different sub-tasks.
    % **MURMUR**发现data-to-text任务直接提示LLM推理易导致幻觉，而提示CoT推理缺乏推理步骤之间的明确条件，损害正确性，并且以不同的顺序线性化数据易造成较大的方差。
    MURMUR~\cite{saha-etal-2023-murmur} notices that prompting CoT reasoning lacks explicit conditioning between inference steps, proposes to first select the potentially correct models at each step, and then select the best model based on the score model.
    % 因此MURMUR提出首先依据预先定义的语法规则在每一步使用束搜索算法选择可能正确的模型范围，再根据打分模型选择最好的模型，以及相应的输入形式。
    % **CHAIN-OF-TABLE**则为了降低单跳LLM上下文学习的难度，提供给LLM预定义的表格操作，需要LLM从中选择一种操作并执行构成操作链。
    ChainHAIN-ofOF-tableTABLE~\cite{anonymous2023chainoftable}, to reduce the difficulty of single-hop reasoning, provides predefined table operations, from which LLMs are required to select one operation and execute.
    
    % 设计prompt的方法和通过prompt分解推理过程的方法并不冲突，二者可以组合使用，具体为在通过prompt分解推理过程后，可以为每一步设计各自的prompt，这样可以分步设计prompt增强模型的表格推理性能。
    The methods of single-step reasoning prompt and multi-step reasoning prompt do not conflict, and the two can be used in combination.
    Specifically, after prompting LLM to decompose the reasoning process, respective prompts can be designed for each step, so that prompt can be designed step by step to enhance the table reasoning performance of the model.
    
\subsection{Tool Learning}
\label{subsec:invoking tools}
    % 目前的研究工作主要分为两条研究思路：一种LLM调用的工具是已经写好并封装的,LLM只需生成调用工具的代码，另一种需要LLM分析需求后，根据具体需求生成代码，比如python、SQL等来实现某一模块或工具的功能。
    The current research is mainly divided into two research ideas: 
    \textit{1}. \textbf{tool using}, which refers to LLM using available tools, and 
    \textit{2}. \textbf{tool making}, which refers to LLM designing tools according to the demand and then using them. 
    % 关于直接调用封装工具的工作，**StructGPT**观察到结构化数据的数量过于庞大，很难全部输入，所以提供了抽取数据的接口，模型通过调用相应接口获得有效数据，再将其输入模型进行推理。
    Regarding the work of tool using, StructGPT~\cite{jiang-etal-2023-structgpt} observes that the amount of structured data is too large to input, so it provides interfaces to extract data, and the model obtains valid data by calling the appropriate interfaces.
    % **Agent**为了同时探索并进一步评估LLM智能体采取行动和推理的能力，提出长对话的数据库问答任务，LLM需要先根据历史进行推理，决定与外部模型的交互策略，再采取行动生成具体的交互命令以调用模型。
    \cite{nan2023db_agent}, to explore and evaluate the action and reasoning capacities of LLM, proposes the long-form database question answering task, where LLMs need to decide an interaction strategy by reasoning, and then generate interaction commands to invoke the external model.
    % **API**在将表格问题翻译成程序后，通过调用其它LLM的API实现了查询知识以及对表格执行程序以外的操作。
    To extend the model capabilities of various TableQA tasks, \cite{cao-etal-2023-api} enables querying knowledge and performing extra tabular operations by calling other LLM APIs.

    % 关于需要LLM根据需求实现工具功能的工作，**BINDER**注意到神经系统缺少可解释性，而符号方法被符号语言的语法限制，但现有的融合方法只针对特定模型和语言，且需要大量训练数据，因此提出首先解析问题中不可以转换成目标程序语言的部分，将其调用大模型的API求解，再将生成结果集成到编程语言中。
    Regarding the work of tool making, Binder~\cite{binder}, noting that existing neural-symbolic works are model- and language-specific and require large training data, proposes to parse the sub-question that are not translatable into the program, invoke the LLM to solve the sub-question.
    % **ReAcTable**注意到根据问题对任意表及其列自动转化的挑战性，提出通过每一步令LLM选择生成不同形式的代码，并调用此代码得到中间结果的表格，来逐步得到答案。
    Observing the challenge of automatically transforming an arbitrary table according to the question, ReAcTable~\cite{zhang2023reactable} proposes to get the answer step by step by making LLM generate a function at each step and calling this code function to get an intermediate table.
    
    % LLM既可以调用现成的函数，也可以先生成代码接口再调用，可以被同时用在LLM的推理过程中，具体为提供部分函数接口，LLM在推理时自动判断调用已有接口或另外生成函数再调用。这样，工具运用更加灵活。
    These two methods of using tools and making tools are not conflicting and can be used simultaneously in the reasoning process of LLM. 
    Specifically to provide some function interfaces, LLM in the reasoning automatically determines to call the existing interface or generate other functions, making the tool learning more flexible.

\subsection{Results Ensemble}
\label{subsec:robustness improvement}
    % 现有的结果集成的方法可以分为两类：如何获得一个问题的多个结果，以及如何在LLM生成的多个结果中选择最有可能的正确结果
    Existing methods of results ensemble mainly focus on two problems: 
    \textit{1}. how to \textbf{obtain multiple results} for a question, and 
    \textit{2}. how to \textbf{select the correct result} among the multiple results.
    % **SQLPrompt**注意到在固定prompt的情况下，LLM生成结果的多样性较差，导致生成结果可能集中于特定的错误答案。
    % 为了解决这个问题，SQLPrompt提出根据多个prompt分别生成结果，然后集成，从而避免生成答案集中于特定结果。
    Considering the work of obtaining multiple results, SQLPrompt~\cite{sun-etal-2023-sqlprompt}, notes that the low diversity of results with fixed prompt and model causes results could be focused on specific incorrect answers, so proposes to generate results with multiple prompts and models.
    % 依照该设计思路，**Lever**专门训练一个打分器对每个生成的答案进行打分，选择相应分数最高的答案作为结果。
    Regarding the work of selecting the correct result, Lever~\cite{ni2023lever} specifically trains a verifier to score each generated answer and selects the answer with the highest score as the result. 
    % Re-rank为了从LLM生成的多个候选SQL中选出正确的，提出在没有正确答案的情况下通过生成新的数据库和用LLM预测执行结果构建test cases，令test cases可以区分所有在原始数据库上有不同执行结果的SQL
    To select the correct from multiple candidate SQL queries, \cite{li2024using_rerank} proposes to construct test cases by generating new databases and using LLM to predict the execution results so that the test cases can distinguish all SQL with different execution results.

    % 这两种问题分别体现在结果集成的两阶段，其中多个结果是选择的基础
    These two problems are respectively reflected in the two stages of the results ensemble, where obtaining multiple results is the basis for result selection.
    % 所以这两种方法可以一起使用，进一步提升模型的表格推理性能
    Therefore, these two problems can be focused on together to further improve the table reasoning performance of the LLM.

% 分析五个方向前人工作多少，原因
\subsection{Comparison}
    \begin{figure}
        \centering
        \input{tex/fig/method_distribution}
        \caption{
            The distribution of the current methods.
        }
        \label{fig:method_distribution}
    \end{figure}
    % 为了帮助研究者思考从哪种方法角度提升模型的表格推理性能更好，我们在这一节统计了现有方法的分布，并横向对比了这5种分类下的现有工作
    To help researchers think about which method to enhance the table reasoning performance is better, we count the distribution of existing methods under five categories as shown in Fig~\ref{fig:method_distribution} and horizontally compare the five method categories in this subsection.
    % 可以发现，研究鲁棒性提升的工作在所有工作中占比最小，因为这一类工作需要集成LLM生成的多个答案，相比较其他方法对时间的开销更大，因此较少有人关注通过提升鲁棒性提升模型表格推理的性能
    The work on results ensemble accounts for the smallest proportion of all work because this type of work requires generating multiple answers by LLMs, which is more time-intensive than other methods, so fewer people pay attention to this method category~\cite{aggarwal-etal-2023-selfconsistency_efficiency}.
    % 而工具学习的工作占比第二少，因为工具学习对模型的能力要求较高，这为表格推理任务带来了新的挑战
    The proportion of tool learning work is the second smallest because tool learning requires higher model capabilities, which could bring new challenges to table reasoning tasks~\cite{cai2023toolmakers}.
    
    % 而模块化分解和上下文学习方法对模型没有较高的要求，而且时间和资源的开销较小，带来的性能提升超过了经过有监督微调的LLM，因此，模块化分解和上下文学习方法的工作在表格推理研究中最多
    The modular decomposition and prompt design methods do not have high requirements on the model, the time overhead is small, and the performance improvement they bring exceeds that of supervised fine-tuning~\cite{gao2023dail,zhang2023tablellama}. 
    Therefore, the works of the modular decomposition and prompt design methods are the most common among table reasoning studies.

==> old_version/6.discussion.tex <==
\begin{table}[t]
    \centering
    \begin{tabular}{l|cc}
        \toprule
        \textbf{Dataset} & \textbf{pre-LLM} & \textbf{LLM few-shot}\\
        \midrule
        % WikiTQ & $0.63$~\cite{jiang-etal-2022-omnitab} & \bm{$0.68$}~\cite{zhang2023reactable} \\
        \multirow{2}{*}{WikiTQ} & $0.63$ & \bm{$0.68$} \\
        ~ & \cite{jiang-etal-2022-omnitab} & \cite{zhang2023reactable} \\
        % TabFact & $0.85$~\shortcite{zhao-yang-2022-tablefact_plm_lka} & \bm{$0.93$}~\shortcite{dater} \\
        \multirow{2}{*}{TabFact} & $0.85$ & \bm{$0.93$} \\
        ~ & \cite{zhao-yang-2022-tablefact_plm_lka} & \cite{dater} \\
        % FeTaQA & $0.65$~\shortcite{xie-etal-2022-unifiedskg} & \bm{$0.71$}~\shortcite{zhang2023reactable} \\
        \multirow{2}{*}{FeTaQA} & $0.65$ & \bm{$0.71$} \\
        ~ & \cite{xie-etal-2022-unifiedskg} & \cite{zhang2023reactable} \\
        % Spider & $0.80$~\shortcite{resdsql} & \bm{$0.87$}~\shortcite{gao2023dail} \\  
        \multirow{2}{*}{Spider} & $0.80$ & \bm{$0.87$} \\
        ~ & \cite{resdsql} & \cite{gao2023dail} \\
        \bottomrule
    \end{tabular}
    \caption{The SOTA methods of pre-LLM and LLM with few-shot on different table reasoning datasets. The WikiTQ refers to the WikiTableQuestions. The evaluation metric for WikiTableQuestions/TabFact/FeTaQA/Spider is accuracy/accuracy/ROUGE-1/execution accuracy.}
    \label{tab:sota}
\end{table}
% 我们以Structure Understanding挑战和Schema Linking挑战为例，在本节分析了LLM本身的特性对解决表格推理挑战的帮助，以便研究者更加充分利用这种能力来解决表格推理挑战以进一步提升性能
LLMs surpass pre-LLMs (Table~\ref{tab:sota}) in tackling table reasoning. 
We analyze the key insights behind this from structure understanding and schema linking perspectives.

\subsection{Structure Understanding}
% 
    % Structure Understanding是指模型能够理解database schema, conversation context and their relationships
    Structure understanding means that the model can understand the table schema, conversation context, and their relationships \cite{unisar}, which poses the key evidence and necessary context information for decoding.
    
    % 相比较PLM，LLM更具有解决理解表格的能力，主要有以下两个原因
    Compared with PLM, LLM can solve the challenge of structure understanding better, mainly for the following two reasons.
    % 1. 因为结构理解和代码理解具有一定的相似性，比如结构理解和代码理解都需要模型识别多层级的索引结构等，而LLM在代码数据上做过训练，对代码理解任务更擅长，所以LLM可以将表格理解任务转换成代码理解任务以获得更好的表现
    1. The code parsing ability LLMs excel at could benefit table understanding ability because both require recognizing the hierarchical structure from plain input (e.g., linearized table to structured table, contextualized code to structured code) \cite{cao-etal-2023-api}.
    % 2. LLM的空间理解能力有助于模型理解结构化表格，都需要根据线性的输入描述想象成二维空间结构
    2. The spatial understanding capabilities of LLM help the model understand structured tables, which both need to be imagined into a two-dimensional spatial structure based on linear descriptions \cite{bubeck2023sparks_gpt4}.

    % 1. The code parsing ability (LLMs excel at) could be shifted (or benifit?) into table understanding ability, which both requires recognizing the hierarchical structure(?) from plain input (e.g., linearized table to structured table, contextualized code to structured code).
    % 我只是展示一个句式，【论点】+【论据】（【argument/statement/hypothesis】+【evidence/proof/intuition】）括号里的英文一一对应，证明强度由强变弱
    % 具体内容可以再推敲，需要保证【简洁】、【自洽】
    
    % 2. 
    
\subsection{Schema Linking}
    % Schema Linking是指将用户问题中出现的实体和表格中的表名、行名和列名对应，减小了问题和schema对应实体间表示的差距，有助于模型在解码时根据问题定位到相关的表格位置
    Schema Linking refers to mapping entities that appear in questions to the columns and tables \cite{guo-etal-2019-schema_linking}, which helps the model locate the positions of relevant cells based on the question when decoding.
    %schema linking回答的问题是"which entities are mentioned by question"， 形式化定义为“align the entity mentions in question with the entity alias in table”
    
    % LLM具有更强的Schema Linking的能力，相比较PLM，主要有以下两个原因
    Compared with PLM, LLMs have stronger capabilities of schema linking, there are two main reasons:
    % 1. LLM具有将问题分解逐步推理来降低推理难度的能力，因此LLM可以通过根据问题分解，在每个分解的子问题中分别寻找与表格中实体的对应完成Schema Linking，相比较针对整个问题进行Schema Linking，针对分解的子问题去掉了问题中与推理和求解不相关的token，能更加专注于实体的链接
    1. LLM can simplify the linking from sentence-level to span-level, via decomposing the complete question and filtering the irrelevant context \cite{din-sql}.
    % 1. LLM can simplify the linking $f$ from sentence-level $f(S,T)$ to span-level $f(R,T)$, where $S$ refers to the whole sentence of user question, $T$ is the table, and $R = \{span_{i} | span_{i} \in S\}$. The ideal schema linking function $\hat f(R, T) = \hat f(S, T), \nexists R' \subseteq R, \hat f(R', T) = \hat f(R, T)$. However $f$ is negatively affected by $S\backslash R$ \cite{din-sql}.
    % 2. Schema Linking需要模型具备常识和广泛的知识，而LLM在知识的泛化性方面比PLM优越很多
    2. The dense commonsense knowledge of LLMs is superior for domain-specific or abbreviation schema linking \cite{liu-etal-2021-awakening}, compared with the sparse knowledge of PLM \cite{yu2023generate_rather_retrieve}.
    

    % 1. simplify the linking from sentence-level to span-level, via decomposing the complext question and filtering the irreleven context. (redundant vs. precise)
    % 2. the dense commonsense knowledge of LLMs is superior for domain-specific or abbreviation schema linking. (sparse vs. dense)

==> old_version/7.future.tex <==
% 为了推动大模型时代的表格推理研究，并且将表格推理应用到实际场景，我们在本节分别从提升LLM表格推理性能，以及扩展实际应用的角度讨论了度讨论表格推理任务未来的研究方向
In order to promote table reasoning research in the LLM era and apply table reasoning to actual scenarios, we discuss the future research directions in this section from both the perspectives of enhancing table reasoning and expanding practical applications.

\subsection{Enhancing Table Reasoning}
    % 我们在本小节按照第3节的分类，分别分析了每个分类下的现有方法不足以及可改进之处
    In this section, we analyze the shortcomings and possible improvements of existing methods under each category in \S\ref{sec:methodology}.
    
    \paragraph{Establishing Diverse Training Data}
        % 由于LLM强大的泛化性，研究者在对LLM有监督微调时应该构建多个表格任务的多样化数据以提升模型在表格推理任务上的总体性能
        Due to the strong generalization of LLM, researchers should construct diverse data for multiple table tasks when performing supervised fine-tuning of LLM to improve the overall performance on table reasoning tasks.
        % 现有方法只是将不同任务的数据简单混合作为训练数据，然而训练数据中不同任务的比重对模型性能有显著影响
        Current pre-existing or manually labeled data methods simply mix diverse data from different table tasks as training data to fine-tune the LLM.
        However, the proportion of different tasks in the training data has a significant impact on model performance.
        % 参考flan工作，我们期待未来工作可以将多个任务的数据以不同的比例混合，探究对模型表格推理能力优化的最佳比重
        Future work should balance the diverse training data from multiple tasks in different proportions to explore the optimal proportion for optimizing the table reasoning capabilities of fine-tuning LLMs \cite{flan}.
    
        % 现有方法只关注数据的某些特征，或特定任务，导致蒸馏的数据并不具有多样性，模型的表格推理性能也无法因此得到全面的提升
        Existing methods of distilled data only focus on certain features or specific tasks, resulting in a lack of diversity in the distilled data, and the table reasoning performance of the model cannot be comprehensively improved by fine-tuning with the distilled data.
        % 因此，未来工作应该使用LLM蒸馏具有不同特征，面向不同任务的多样化数据，以提升模型在表格推理任务上的综合能力以及泛化性。
        Therefore, it is worth exploring how to distill diverse data with different features and for different tasks to improve the LLM comprehensive ability and generalization in table reasoning tasks \cite{xu2023wizardlm,luo2023wizardcoder}.
    
    \paragraph{Improving Results Sampling Efficiently}
        % 为了令集成后可以获得正确的答案，研究者应该关注如何在可能的结果空间中采样可以获得正确答案
        To obtain the correct answer after ensemble, researchers should focus on how to sample in the possible result space effectively.
        % 获取多个结果的主要目的是拓宽采样空间，以使空间中包含更多正确答案
        The main purpose of obtaining multiple results is to widen the sampling space so that more correct answers can be sampled.
        % 但现有关于获取多个结果的工作并没有考虑改变prompt中的demonstration以提升结果的多样化和正确性，而demonstration对模型表格推理结果的影响是显著的
        However, existing works do not consider changing the demonstrations in the prompt to improve the correctness of the results, and the impact of the demonstrations on the table reasoning performance of LLM is significant.
        % 参考CONDACC工作，未来工作应该改变demonstration以获得更加有可能正确的结果
        Future work should change the demonstrations to sample results that are more likely to be correct \cite{chang-jia-2023-data_icl}.
        
        % 现有选择正确结果的工作只依据最终结果，没有考虑到结果个数随着推理步数的增长呈指数增长，在指数大的搜索空间中采样很难采样到正确答案
        Current studies on selecting the correct answer only rely on the final result and do not take into account that the number of results increases exponentially with the growing number of reasoning steps, and it is difficult to sample the correct answer in an exponentially large search space.
        % 参考Self-Evaluation，LLM可以对表格推理的路径做集成，通过选择正确的推理路径减少搜索空间，进一步选出正确答案。
        Future work should make full use of the multi-step reasoning path, narrow the search space by selecting the correct reasoning path at each step, and further select the correct answer \cite{xie2023selfevaluation}.

    \paragraph{Optimizing Prompt Automatically}
        % 由于LLM的性能严重依赖于prompt，研究者应该关注如何根据问题自动优化表格推理的prompt
        Since the performance of LLM relies heavily on prompts, researchers should focus on how to automatically optimize prompts for table reasoning based on the question.
        % 现有研究均是从有限范围内人工比较或设计算法选择更好的prompt作为输入，导致模型性能的提升也是有限的。
        Prompt design research on single-step reasoning compares candidate prompts from a limited range of human-labeled instructions and examples, which results in performance improvement is also limited.
        % 为了更好地设计prompt，参考OPTIMIZERS工作，能够借助LLM自动生成上下文，并根据表格和任务对prompt打分以及优化，更好地帮助模型理解并解决这个问题。
        To design a better prompt, future work should automatically generate the prompt and optimize it with LLMs based on the question and tables \cite{yang2023optimizers}.
        
        % 现有关于多步推理的研究没有考虑到多步推理造成的错误级联问题，造成错误的中间结果导致后续推理的错误
        Existing studies on multi-step reasoning prompts do not consider the error cascade problem in table reasoning and cause erroneous intermediate results leading to errors in subsequent reasoning.
        % 而ToT方法则通过选取多个可能的中间过程及结果缓解了这种问题，那么如何将TOT应用到表格推理任务值得未来关注
        The prompt method of ToT~\cite{yao2023treeofthoughts} alleviates this problem by maintaining multiple possible intermediate steps in multi-step reasoning, so how to apply TOT to table reasoning tasks deserves future attention.
    
    \paragraph{Making Fuller Use of Modular Generation}
        % 基于现有工作，如何充分利用模块化分解针对每个表格推理问题降低其难度以提升总体性能，值得研究者的注意
        Based on existing works, how to make fuller use of modular decomposition to reduce the difficulty of each table reasoning question to improve overall performance deserves the attention of researchers.
        % 现有方法需要人工预先将任务分解，但这种分解只适用于某一类表格任务，并不具有普适性，而固定的适用于所有表格任务的分解又太过概括，并不能很好地降低推理难度。
        Current methods require manually decomposing the task into different modules in advance.
        However, this decomposition can only apply to a certain table task. 
        In contrast, the fixed decomposition applicable to all table tasks is too general and does not reduce the difficulty of reasoning well.
        % 参考Agent，希望能够待无需为LLM解决某一表格问题指定流水线，而是令LLM能够根据问题自主将任务显示分解，能适合于所有表格任务，很好地降低单步推理难度并且减少人工参与。
        Therefore, instead of specifying the decomposition for a particular table task, future work should automatically decompose the task according to the question, which is suitable for all table tasks without human involvement and greatly reduces the difficulty of single-step reasoning \cite{yao2023react}.

        % 对于工具学习的工作，现有工作没有注意到生成的函数本身也有可能错误，为表格推理过程引入额外的错误
        For the methods of tool learning, current works do not notice that the generated function may be wrong, causing extra errors in the table reasoning process.
        % 参考tool maker，未来工作应该在工具制作之后加入工具验证过程，以保证生成的工具可以被正确应用
        Future work should include a tool verification process after the tool making to ensure that the generated tool can be applied correctly in the table reasoning task \cite{cai2023toolmakers}.
        
        % 现有方法中从海量表格获取数据，即检索器和基于表格推理回答问题，即生成器的关系较为独立，检索很有可能返回不相关表格并导致推理错误
        In existing open-domain methods, the retriever that obtains data from massive tables and the generator that generates answers based on table reasoning is relatively independent, and retrieval could return irrelevant tables and further lead to reasoning errors.
        % 因此，如何利用生成器的结果反馈给检索器，以增强检索器的性能值得未来工作的关注，因为生成的结果可以用来判断检索到的表格是否与问题相关并修改检索查询
        Therefore, to enhance the performance of the retriever, it is worth exploring utilizing the results of the generator to provide feedback on the retriever in future works because the generated results can be used to determine whether the retrieved tables are relevant to the question and further modify the retrieval query \cite{shao-etal-2023-retrieval-augmented}.
    

    
    \paragraph{Exploring Reliable Tools}
        % 合作工具会帮助模型解决本身难以解决的子任务，但为了保证工具本身不会引入额外的错误，未来工作应该探索更加可信赖的工具以更好地帮助模型表格推理
        Collaborating with tools helps the model solve sub-tasks that are difficult to solve by itself, but to ensure that the tools do not introduce additional errors, future work should explore more reliable tools to better assist model table reasoning.
        % 现有研究没有关注到表格推理任务中面临的知识密集场景，而调用LLM查询知识又容易产生幻觉，不能灵活运用外部数据进行知识注入。
        Current works of tool using do not focus on the knowledge-intensive scenarios faced in table reasoning tasks, and calling LLM to query knowledge is prone to hallucinations.
        % and cannot flexibly use external data sources for knowledge injection.
        % 参考WebGPT，我们希望处理专家问题时LLM能够自主借助搜索引擎查询相关领域内知识，并且将查询结果用于计算或推理。
        To use reliable external data sources for knowledge injection, future work should query relevant domain knowledge with the search engine and utilize the queried knowledge for reasoning when dealing with expert problems \cite{nakano2022webgpt}.
    
        % 对于工具制作的工作，现有工作没有注意到生成的函数本身也有可能错误，为表格推理过程引入额外的错误
        For the methods of tool making, current works do not notice that the generated function may be wrong, causing extra errors in the table reasoning process.
        % 参考tool maker，未来工作应该在工具制作之后加入工具验证过程，以保证生成的工具可以被正确应用
        Future work should include a tool verification process after the tool making to ensure that the generated tool can be applied correctly in the table reasoning task \cite{cai2023toolmakers}.



\paragraph{Multi-Modal}
    % (xxx是什么)
    % (为什么需要研究xxx/xxx如何推进现有的tabel reasoning的应用)
    % (LLM时代，如何增强表格相关的xxx)
    % 多模态任务是指the process of automated understanding, classifying, and extracting information with rich typesetting formats from textual, visual and other types evidence.
    The multi-modal setting requires the model to encompass automated comprehension, classification, and extraction of information from textual, visual, and other forms of evidence \cite{cui2021documentai}.
    % 因为现实场景中有很多表格以图片的形式存储，直接OCR会因为识别错误带来信息损失，所以我们需要结合视觉模型更好地理解和推理图片表格
    Because there are many tables stored in the form of images in actual scenarios, direct Optical Character Recognition (OCR) will cause information loss due to the recognition errors, so we need to combine visual models to better understand and reason about image tables.
    % 因为语言模型输入表格需要将其转为序列破坏了二维结构，而视觉模型可以接收二维输入，保留了表格的结构信息，所以结合视觉模型能更好地理解和处理表格
    % For the table reasoning task, the combination of the visual model can better understand and process the table, since the language model can only accept one-dimensional input, while the visual model can receive two-dimensional input, retaining the structure information.
    % 为了更好地对齐自然语言问题与视觉图表信息，未来研究可以探索设计结构，来将问题中的实体与图片表格中的表头对齐，增强图片与文本间的语意对齐
    To better align natural language questions and visual information, future research can explore design structures to align entities in questions with headers in image tables, thereby enhancing semantic alignment between images and text \cite{anonymous2024minigpt}.

\paragraph{Agent}
    % An agent refers to an entity capable of perceiving its environment, making decisions, and taking actions （paraphrase一下）
    The agent method denotes equipping with the capabilities to perceive the surrounding environment, engage in decision-making processes, and execute actions based on these decisions \cite{xi2023agent_survey}.
    % 由于在现实场景中，当LLM面对复杂的表格推理问题难以独自解决时，可以与其它agent合作，比如代码、搜索引擎等
    In real scenarios, when LLM faces complex table reasoning problems that are difficult to solve alone, it can cooperate with other agents, such as code, search engines.
    % 因为不同的agent适合解决不同的问题，不同的agent对同一问题带来的性能改变也是不同的，为了进一步提升表格推理的性能，未来研究可以通过探索更多适合不同表格任务的agent增强表格推理任务与agent的合作
    Because different agents are suitable for solving different tasks, and different agents bring different performance changes to the same task, future research can enhance cooperation with agents by exploring more diverse agents suitable for different table tasks in actual scenarios \cite{cao-etal-2023-api}.

\paragraph{Dialogue}
    % Dialogue systems perform chit-chat with human or serve as an assistant via conversations.
    Dialogue systems are designed to converse with humans as assistants through conversational interactions \cite{dialogue_survey}.
    % 由于与用户交互的过程中，可能存在模型返回结果错误、用户问题表达不清的问题，导致需要多轮交互来纠正错误，因此需要增强模型针对chat的table reasoning能力
    During the process of interacting with users, there could be problems such as incorrect model results and ambiguous questions, which require multiple turns of interactions to correct errors. 
    Therefore, it is necessary to enhance the table reasoning ability with dialogues.
    % 在表格推理任务中模型需要根据表格和用户提出的问题focus on相关的子表，尤其在面对庞大的表格时，而在多轮对话时，这种问题相关的子表是不断变化的
    When reasoning based on tables, the model needs to focus on the sub-tables that are related to the user question, especially when facing huge tables \cite{dater}. 
    % 未来研究应该关注如何迭代地高效利用子表，如果问题是基于之前轮次的问题的追问，可以直接使用之前轮次分解的表格继续推理，提升了多轮表格对话的效率和推理的准确性 回溯
    During multiple turns of dialogues, the question-related sub-tables are constantly changing, so future work should study how to backtrace the sub-tables decomposed previously to obtain the whole relevant information, preventing that the last sub-table does not include the required information in the turn \cite{yao2023treeofthoughts}.

\paragraph{Retrieval-Augmented Generation}
    % RAG refers to the model when answering questions or generating text, first retrieving relevant information from a vast corpus of documents.
    Retrieval-Augmented Generation (RAG) technology denotes retrieving the reasoning-related information from a large number of documents before the reasoning \cite{gao2024rag_survey}.
    % 由于在应用中表格推理任务中经常面临知识密集场景，而LLM缺乏领域内知识，所以未来工作应该关注基于检索知识增强模型的领域内表格推理能力
    Since the table reasoning task often faces knowledge-intensive scenarios in applications where the in-domain knowledge of LLM is not sufficient to solve, future work should focus on enhancing table reasoning capabilities with retrieving knowledge \cite{dou-etal-2022-knowledge-intensive}.
    % 表格推理任务中，会面临LLM不了解实体含义以致模型难以理解表格，导致模型很难正确回答用户问题的挑战，为了解决这一挑战，未来研究应该关注根据表格中的实体检索来增强
    In table reasoning tasks, LLM could be challenging to understand the meaning of some entities in the table, making it difficult for the model to understand the meaning of the table, thereby correctly answering the user question \cite{liu-etal-2021-awakening}. 
    To solve this challenge, future research should detect the unknown entities in the table to better retrieve the related information.












% \paragraph{Privacy and security}
%     % https://arxiv.org/pdf/2205.10095.pdf
%     % Privacy is the ability to control the extent of personal matters an individual wants to reveal
%     % 由于在实际场景中使用大模型进行表格推理时，某些表格中的敏感信息无法直接输入给模型，因此模型需要有根据脱敏后的表格进行正确table reasoning的能力
%     % 

% 为了启发未来研究，在本节，我们将介绍如何改进各类方法，来提升LLM的表格推理能力。
% To inspire future research, we discuss how to improve LLM capacities for table reasoning under different method categories in this section.


    


==> old_version/mind_mapping.tex <==
% \tikzset{%
%     parent/.style = {align=center,text width=2.0cm,rounded corners=3pt, line width=0.3mm, fill=white!10,draw=gray!80, minimum height=0.3cm, anchor=center},
%     sft/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=white!10,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},  
%     sft_div/.style = {align=center,text width=3.6cm,rounded corners=3pt, fill=cyan!3,draw=cyan!15,line width=0.1mm, minimum height=0.3cm, anchor=center}, 
%     sft_work/.style = {align=left, text width=6.0cm,rounded corners=3pt, fill=cyan!10,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},  
%     md/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=white!10,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},
%     md_work/.style = {align=left,text width=6.0cm,rounded corners=3pt, fill=cyan!10,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},
%     icl/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=white!10,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},
%     icl_div/.style = {align=center,text width=3.6cm,rounded corners=3pt, fill=cyan!3,draw=cyan!15,line width=0.1mm, minimum height=0.3cm, anchor=center},
%     icl_work/.style = {align=left,text width=6.4cm,rounded corners=3pt, fill=cyan!10,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},
%     it/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=white!10,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},   
%     it_div/.style = {align=center,text width=3.6cm,rounded corners=3pt, fill=cyan!3,draw=cyan!15,line width=0.1mm, minimum height=0.3cm, anchor=center},
%     it_work/.style = {align=left,text width=6.0cm,rounded corners=3pt, fill=cyan!10,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},
%     ri/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=white!10,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},   
%     ri_work/.style = {align=left,text width=5.6cm,rounded corners=3pt, fill=cyan!10,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},
% }
\tikzset{
    parent/.style = {align=center,text width=2.0cm,rounded corners=3pt, line width=0.3mm, fill=customColor,draw=gray!80, minimum height=0.3cm, anchor=center},
    sft/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=customColor,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},  
    sft_div/.style = {align=center,text width=3.6cm,rounded corners=3pt, fill=customColor,draw=cyan!15,line width=0.1mm, minimum height=0.3cm, anchor=center}, 
    sft_work/.style = {align=left, text width=6.0cm,rounded corners=3pt, fill=customColor,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},  
    md/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=customColor,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},
    md_work/.style = {align=left,text width=6.0cm,rounded corners=3pt, fill=customColor,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},
    icl/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=customColor,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},
    icl_div/.style = {align=center,text width=3.6cm,rounded corners=3pt, fill=customColor,draw=cyan!15,line width=0.1mm, minimum height=0.3cm, anchor=center},
    icl_work/.style = {align=left,text width=6.4cm,rounded corners=3pt, fill=customColor,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},
    it/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=customColor,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},   
    it_div/.style = {align=center,text width=3.6cm,rounded corners=3pt, fill=customColor,draw=cyan!15,line width=0.1mm, minimum height=0.3cm, anchor=center},
    it_work/.style = {align=left,text width=6.0cm,rounded corners=3pt, fill=customColor,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},
    ri/.style = {align=center,text width=2.7cm,rounded corners=3pt, fill=customColor,draw=gray!80,line width=0.1mm, minimum height=0.3cm, anchor=center},   
    ri_work/.style = {align=left,text width=5.6cm, rounded corners=3pt, fill=customColor,draw=cyan!40,line width=0.1mm, minimum height=0.3cm, anchor=center},
}

\begin{forest}
    for tree={
        forked edges,
        grow'=0,
        draw,
        rounded corners,
        s sep=4pt,
        align=center
    },
    [Table Reasoning Task, parent
        % sft
        [Supervised Fine-Tuning \S~\ref{subsec:supervised fine-tuning}, for tree={sft}
            % [fine-tuning based on pre-existing datasets, sft_div
                % [TabLLM~\cite{pmlr-v206-tabllm}; TableGPT~\cite{zha2023tablegpt};\\TableLlama~\cite{zhang2023tablellama}; APEL~\cite{zhong-etal-2023-apel};\\TaCo~\cite{zheng-etal-2023-taco}, sft_work]
            [{\begin{tabular}[t]{@{}l@{}}TabLLM~\cite{pmlr-v206-tabllm}; TableGPT~\cite{zha2023tablegpt};\\TableLlama~\cite{zhang2023tablellama}; APEL~\cite{zhong-etal-2023-apel};\end{tabular}}, sft_work]
            % ]
            % [fine-tuning based on distilled data, sft_div
            [\cite{yang2023distill}; HELLaMa~\cite{bian2023hellama}, sft_work]
            % ]
        ]
        % md
        [Modular Decomposition \S~\ref{subsec:modular decomposition}, for tree={md}
            % [DATER~\cite{dater}; DIN-SQL~\cite{din-sql}; TableQAKit~\cite{lei2023tableqakit};\\CRUSH4SQL~\cite{kothyari-etal-2023-crush4sql}; OpenTab~\cite{anonymous2023opentab}; DBCopilot~\cite{wang2023dbcopilot};\\MAC-SQL~\cite{wang2023macsql}, md_work]
            [{\begin{tabular}[t]{@{}l@{}}DATER~\cite{dater}; DIN-SQL~\cite{din-sql};\\TableQAKit~\cite{lei2023tableqakit}\end{tabular}}, md_work]
            [{\begin{tabular}[t]{@{}l@{}}CRUSH4SQL~\cite{kothyari-etal-2023-crush4sql}; OpenTab~\cite{anonymous2023opentab};\\DB-GPT~\cite{xue2024dbgpt}; DBCopilot~\cite{wang2023dbcopilot};\\MAC-SQL~\cite{wang2023macsql};\end{tabular}}, md_work]
        ]
        % icl
        [Prompt Design \S~\ref{subsec:in-context learning}, for tree={icl}
            % [designing prompt, icl_div
                % [\cite{chen-2023-few}; ODIS~\cite{chang-fosler-lussier-2023-selective_odis};\\DAIL-SQL~\cite{gao2023dail}; SEER~\cite{tonglet-etal-2023-seer};\\\cite{nan-etal-2023-enhancing}; \cite{zhao-etal-2023-parseres};\\TAP4LLM\cite{sui2023tap4llm}; Auto-CoT~\cite{zhang2023actsql_autocot}, icl_work]
            [{\begin{tabular}[t]{@{}l@{}}\cite{chen-2023-few}; ODIS~\cite{chang-fosler-lussier-2023-selective_odis};\\DAIL-SQL~\cite{gao2023dail}; SEER~\cite{tonglet-etal-2023-seer};\\\cite{nan-etal-2023-enhancing}; \cite{zhao-etal-2023-parseres}; TAP4LLM\cite{sui2023tap4llm};\\Auto-CoT~\cite{zhang2023actsql_autocot}\end{tabular}}, icl_work]
            % ]
            % [decomposing reasoning via prompt, icl_div
            [MURMUR~\cite{saha-etal-2023-murmur}; CHAIN-OF-TABLE~\cite{anonymous2023chainoftable}, icl_work]
            % ]
        ]
        % it
        [Tool Learning \S~\ref{subsec:invoking tools}, for tree={it}
            % [calling wrapper tools, it_div
            [StructGPT~\cite{jiang-etal-2023-structgpt}; \cite{nan2023db_agent}; \cite{cao-etal-2023-api}, it_work]
            % ]
            % [implementing tool functionality, it_div
            [Binder~\cite{binder}; ReAcTable~\cite{zhang2023reactable}, it_work]
            % ]
        ]
        % ri
        [Results Ensemble \S~\ref{subsec:robustness improvement}, for tree={ri}
            [SQL-Prompt~\cite{sun-etal-2023-sqlprompt}, ri_work]
            [Lever~\cite{ni2023lever}; \cite{li2024using_rerank}, ri_work]
        ]
    ]
\end{forest}


==> tex/fig/method_distribution.tex <==
% \resizebox{\linewidth}{!}{
%     \begin{tikzpicture}[scale=0.6]
%         \pie[
%             pos={8,0},
%             explode=0.1,
%             color={blue!15, blue!30, blue!45, blue!60},
%             text=legend
%         ]{
%             10/Table Understanding,
%             20/Heterogeneous Modeling,
%             30/Information Extraction,
%             40/Multi-Hop Reasoning
%         }
%     \end{tikzpicture}
% }

% \resizebox{0.9\linewidth}{!}{
%     \begin{tikzpicture}[scale=0.6]
%         \small
%         \pie[
%             pos={8,0},
%             explode=0.1,
%             color={cyan!10, cyan!20, cyan!30, cyan!40, cyan!50},
%             text=legend
%         ]{
%             9.1/Results Ensemble,
%             15.2/Tool Learning,
%             21.2/Supervised Fine-tuning,
%             24.2/Modular Decomposition,
%             30.3/Prompt Design
%         }
%     \end{tikzpicture}
% }

\resizebox{0.9\linewidth}{!}{
    \begin{tikzpicture}[scale=0.6]
        \small
        \pie[
            pos={8,0},
            color={baseColor!20, baseColor!90, baseColor!160, baseColor!230, baseColor!300},
            text=legend
        ]{
            6.67/Step-by-Step Reasoning (2),
            10.00/Result Ensemble (3),
            16.67/Supervised Fine-tuning (5),
            23.33/In-Context Learning (7),
            43.33/Instruction Following (13)
        }
    \end{tikzpicture}
}

